Symmetry Abstractions for Hybrid Systems and their Applications

A symmetry of a dynamical system is a map that transforms one trajectory to another trajectory. We introduce a new type of abstraction for hybrid automata based on symmetries. The abstraction combines different modes in a concrete automaton A, whose trajectories are related by symmetries, into a single mode in the abstract automaton B. The abstraction sets the guard and reset of an abstract edge to be the union of the symmetry-transformed guards and resets of the concrete edges. We establish the soundness of the abstraction using a forward simulation relation (FSR) and present several examples. Our abstraction results in simpler automata, that are more amenable for formal analysis and design. We illustrate an application of this abstraction in making reachability analysis faster and enabling unbounded time safety verification. We show how a fixed point of the reachable set computation of B can be used to answer reachability queries for A, even if the latter visits an infinite and unbounded sequences of modes. We present our implementation of the abstraction construction, the fixed point check, and the map that transforms abstract reachable sets to concrete ones in a software tool. Finally, we show the advantage of our method over existing ones, and the different aspects of our abstraction, in a sequence of experiments including scenarios with linear and nonlinear agents following waypoints.

==> acknowledgment.tex <==
\section{Acknowledgments}
\label{sec:ack}
%\vspace{-.15in}
The authors are supported by a research grant from The Boeing Company and a research grant from NSF (CPS 1739966). We would like to thank John L. Olson and Arthur S. Younger from The Boeing Company for valuable technical discussions.
\vspace{-.2in}



==> exp_results.tex <==
\subsection{Setup and results}


==> inf_initset.tex <==
\subsection{Reachtubes starting from Infinite Initial Sets}
\label{sec:inf_initset}


==> prelude.tex <==
% !TEX root = main.tex
% marking changes

%\newcommand{\mitras}[1]{\textcolor{blue}{#1}}
\newcommand{\mitras}[1]{{#1}}
% for nomencl to produce page links
%\renewcommand*{\pagedeclaration}[1]{\unskip, \hyperpage{#1}}
%\renewcommand{\nomname}{List of Symbols and Functions}

\newcommand{\authcomment}[1]{\textbf{[[#1]]}}
\newcommand{\sayan}[1]{\textcolor{blue}{#1}}


%FIXED SETS

%\newcommand{\Time}{{\sf T}}                     %time domain
\newcommand{\nnt}{{\sf T}^{\geq 0}}             %nonnegative time points
\newcommand{\post}{{\sf T}^{>0}}                %positive time points
\newcommand{\Variables}{{\sf V}}                %variables

\newcommand{\num}[1]{\relax\ifmmode \mathbb #1\else $\mathbb #1$\fi}
\newcommand{\nnnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\geq 0} \else ${\mathbb #1}_{\geq 0}$
  \fi}
\newcommand{\npnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\leq 0} \else ${\mathbb #1}_{\leq 0}$
  \fi}
\newcommand{\pnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{> 0} \else ${\mathbb #1}_{> 0}$
  \fi}
\newcommand{\nnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{< 0} \else ${\mathbb #1}_{< 0}$
  \fi}
\newcommand{\plnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{+} \else ${\mathbb #1}_{+}$
  \fi}
\newcommand{\nenum}[1]{\relax\ifmmode 
  {\mathbb #1}_{-} \else ${\mathbb #1}_{-}$
  \fi}

\newcommand{\bools}{{\num B}}                    %reals
\newcommand{\reals}{{\num R}}                    %reals
\newcommand{\nnreals}{{\nnnum R}}                    %nonnegative reals
\newcommand{\realsinfty}{{\num R} \cup \{\infty, -\infty\}}                    %nonnegative reals
\newcommand{\plreals}{{\plnum R}}                    %positive reals
\newcommand{\naturals}{{\num N}}                      %natural numbers
\newcommand{\integers}{{\num Z}}                      %integers
\newcommand{\nnintegers}{{\nnnum Z}}    
\newcommand{\rationals}{{\num Q}}                      %rationals
\newcommand{\nnrationals}{{\nnnum Q}}                   % nonnegative rationals
\newcommand{\Time}{{\num T}}  


\newcommand{\R}{\mathbb{R}}

% ************** Sayan's New definitions will be added in this block START
% EXECUTIONS TRACES and FRAGS
\newcommand{\extb}[1]{\relax\ifmmode {\sf ExtBeh}_{#1} \else ${\sf ExtBeh}_{#1}$\fi} 
\newcommand{\tdists}[1]{\relax\ifmmode {\sf Tdists}_{#1} \else ${\sf Tdists}_{#1}$\fi} 

\newcommand{\exec}[1]{\relax\ifmmode {\sf Execs}_{#1} \else ${\sf Execs}_{#1}$\fi} 
\newcommand{\execf}[1]{\relax\ifmmode {\sf Execs}^*_{#1} \else ${\sf Execs}^*_{#1}$\fi} 
\newcommand{\execi}[1]{\relax\ifmmode {\sf Execs}^\omega_{#1} \else ${\sf Execs}^\omega_{#1}$\fi} 

\newcommand{\fintrace}[1]{\relax\ifmmode {\sf FinTraces}_{#1} \else ${\sf FinTraces}_{#1}$\fi} 

\newcommand{\trace}[1]{\relax\ifmmode {\sf Traces}_{#1} \else ${\sf Traces}_{#1}$\fi} 
\newcommand{\tracef}[1]{\relax\ifmmode {\sf Traces}^*_{#1} \else ${\sf Traces}^*_{#1}$\fi} 
\newcommand{\tracei}[1]{\relax\ifmmode {\sf Traces}^\omega_{#1} \else ${\sf Traces}^\omega_{#1}$\fi} 

\newcommand{\frag}[1]{\relax\ifmmode {\sf Frags}_{#1} \else ${\sf Frags}_{#1}$\fi} 
\newcommand{\fragf}[1]{\relax\ifmmode {\sf Frags}^*_{#1} \else ${\sf Frags}^*_{#1}$\fi} 
\newcommand{\fragi}[1]{\relax\ifmmode {\sf Frags}^\omega_{#1} \else ${\sf Frags}^\omega_{#1}$\fi} 

\newcommand{\reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi} 


\newcommand{\ball}[1]{\relax\ifmmode {\mathit{B}}_{#1} \else ${\mathit{B}}_{#1}$\fi} 

\newcommand{\untimexec}[1]{\relax\ifmmode {\sf Untimexecs}_{#1} \else ${\sf Untimexecs}_{#1}$\fi} 

\newcommand{\untimexecs}{{\untimexec{}}}
\newcommand{\execs}{{\exec{}}}
\newcommand{\traces}{{\trace{}}}
\newcommand{\fragss}{{\frag{}}}

\newcommand{\fexecs}{{\execf{}}}
\newcommand{\ftraces}{{\tracef{}}}
\newcommand{\ffragss}{{\fragf{}}}

\newcommand{\iexecs}{{\execi{}}}
\newcommand{\itraces}{{\tracei{}}}
\newcommand{\ifragss}{{\fragi{}}}
\newcommand{\tclose}{\relax\ifmmode {\sf tclosure} \else ${\sf tclosure}$\fi} 
\newcommand{\card}{\relax\ifmmode {\sf card} \else ${\sf card}$\fi} 
\newcommand{\tabs}[1]{\relax\ifmmode {\sf Untimed}(#1) \else ${\sf TAbs(#1)}$\fi} 

% lstate fstate
\newcommand{\dom}{\relax\ifmmode {\sf dom} \else ${\sf dom}$\fi} 
\newcommand{\lstate}{\relax\ifmmode {\sf lstate} \else ${\sf lstate}$\fi} 
\newcommand{\fstate}{\relax\ifmmode {\sf fstate} \else ${\sf fstate}$\fi} 
\newcommand{\ltime}{\relax\ifmmode {\sf ltime} \else ${\sf ltime}$\fi} 
\newcommand{\prestate}{\relax\ifmmode {\sf prestate} \else ${\sf prestate}$\fi} 
\newcommand{\poststate}{\relax\ifmmode {\sf poststate} \else ${\sf poststate}$\fi} 


\newenvironment{noqedproof}{\pf}{}
\newcommand{\pf}{\par\noindent{\bf Proof:}~}

% repeating theorems: should come after other theorem definitions
\theoremstyle{box}
\newtheorem{duplicate}{NameIgnored}

% ************** Sayan's New definitions will be added in this block END


 %\newtheorem{theorem}{Theorem}[chapter]
% \newtheorem{lem}{Lemma}
 %\newtheorem{corollary}[theorem]{Corollary}
 %\newtheorem{claim}[theorem]{Claim}
%\theoremstyle{definition}
 %\newtheorem{definition}{Definition}[chapter]
 %\renewcommand{\qed}{\hfill{\rule{2mm}{2mm}}\medskip}
 %\newenvironment{proof}{\pf}{\qed}
 %\newtheorem{proposition}[theorem]{Proposition}
%\newenvironment{inv}{\begin{theorem}}{\end{theorem}}
% \newtheorem{inv}{Invariant}
 \newtheorem{assumption}{Assumption}

 
 %\newenvironment{example}
 %{\refstepcounter{theorem} \vspace{2ex}\par\noindent
 %\textbf{Example}~\textbf{\thetheorem~}}{\qed}
 
%\theoremstyle{remark}
% 
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \newcommand{\Section}[1]{\section{#1}%
%    \setcounter{equation}{0}\setcounter{figure}{0}\setcounter{table}{0}%
%    \setcounter{example}{0}}
% 
% \newenvironment{anotation}[1][Nancy]{\begin{quote}\small[[[#1]]]}{\normalsize\end{quote}}
% \newcommand{\ba}{\begin{anotation}}
% \newcommand{\ea}{\end{anotation}}
% 
% \newcommand{\bcb}{\chgbarbegin}
% \newcommand{\ecb}{\chgbarend}
% \chgbarwidth 1pt
% 
% \newcommand{\dec}{\ensuremath{{:}}}
% \newcommand{\eqdef}{\mathbin{::=}}
% \newcommand{\I}{{\ensuremath{\cap}}}



% OPERATIONS ON SETS, RELATIONS AND FUNCTIONS
\newcommand{\pow}[1]{{\bf P}(#1)} % powerset
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\range}[1]{\mathit{range{(#1)}}}
\newcommand{\domain}[1]{{\mathit dom}(#1)}
\newcommand{\type}[1]{\mathit{type{(#1)}}}
\newcommand{\val}[1]{\mathit{val{(#1)}}}
\newcommand{\dtype}[1]{\mathit{dtype{(#1)}}} % dynamic type
\newcommand{\restr}{\mathrel{\lceil}}
\newcommand{\proj}{\matrel{\lceil}}
\newcommand{\restrrange}{\mathrel{\downarrow}}
\newcommand{\point}[1]{\wp(#1)}     		%point trajectory



% HYBRID AUTOMATA
\def\A{{\bf A}} % HA
\def\B{{\bf B}} % HA
\def\C{{\cal C}} % HA
\def\D{{\bf D}} % set of discrete steps
\def\DC{{\bf DC}} % points of discontinuity
\def\E{{\cal E}} % HA
\def\F{{\cal F}} % HA
\def\G{{\cal G}} % pieces of SHIOA
\def\H{{\cal H}} % HA
\def\I{{\cal I}} % environment sequence
\def\K{{\cal K}} % environment sequence
\def\M{{\cal M}} % Mode switching transitions
\def\O{{\cal O}} % outcome function
\def\P{{\cal P}} % set of modes
\def\Q{{\cal Q}} % set of modes
\def\R{{\cal R}} % relation
\def\S{{\cal S}} % set of trajectories
\def\T{{\bf T}} % set of trajectories
\def\V{{\cal V}} % Lyapunov function
\def\U{{\cal U}} % set of trajectories
\def\X{{\cal X}} % Lyapunov function
\def\Y{{\cal Y}} % set of trajectories


% more special characters

\newcommand{\col}[1]{\relax\ifmmode \mathscr #1\else $\mathscr #1$\fi}

\def\statemodels{\col{S}}

% LTS related

\newcommand{\atpro}{\mathit{AP}}
\newcommand{\stlab}{\mathit{Lab}}


% Names of actions, automata etc
\definecolor{HIOAcolor}{rgb}{0.776,0.22,0.07}
\newcommand{\HIOA}{\textcolor{HIOAcolor}{\tt HIOA\hspace{3pt}}}
\newcommand{\PVS}{\textcolor{HIOAcolor}{\tt PVS\hspace{3pt}}}
\newcommand{\PVSnogap}{\textcolor{HIOAcolor}{\tt PVS\hspace{1pt}}}
\newcommand{\HIOAbiggap}{\textcolor{HIOAcolor}{\tt HIOA\hspace{6pt}}}
\newcommand{\HIOAnogap}{\textcolor{HIOAcolor}{\tt HIOA}}
\newcommand{\anyrelation}{\lessgtr}


% Transformation for ADT
\newcommand{\SC}[2]{\relax\ifmmode {\tt Scount}(#1,#2) \else ${\tt Scount}(#1,#2)$\fi} 
\newcommand{\SCM}[2]{\relax\ifmmode {\tt Smin}(#1,#2) \else ${\tt Smin}(#1,#2)$\fi} 
\newcommand{\Aut}[1]{\relax\ifmmode {\tt Aut}(#1) \else ${\tt Aut}(#1)$\fi} 

\newcommand{\auto}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\act}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\smodel}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\pvstheory}[1]{{\operatorname{\mathit{#1}}}}
%\newcommand{\auto}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}
%\newcommand{\act}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}


\newcommand{\Automaton}{{\bf automaton}}
\newcommand{\Asserts}{{\bf asserts}}
\newcommand{\Assumes}{{\bf assumes}}
\newcommand{\Backward}{{\bf backward}}
\newcommand{\By}{{\bf by}}
\newcommand{\Case}{{\bf case}}
\newcommand{\Choose}{{\bf  choose}}
\newcommand{\Components}{{\bf components}}
\newcommand{\Const}{{\bf const}}
\newcommand{\Converts}{{\bf converts}}
\newcommand{\Do}{{\bf do}}
\newcommand{\Eff}{{\bf eff}}
%\newcommand{\Else}{{\bf else}}
\newcommand{\Elseif}{{\bf elseif}}
\newcommand{\Enumeration}{{\bf enumeration}}
\newcommand{\Ensuring}{{\bf ensuring}}
\newcommand{\Exempting}{{\bf exempting}}
\newcommand{\Fi}{{\bf fi}}
%\newcommand{\For}{{\bf for}}
\newcommand{\Forward}{{\bf forward}}
\newcommand{\Freely}{{\bf freely}}
\newcommand{\From}{{\bf from}}
\newcommand{\Generated}{{\bf generated}}
\newcommand{\Local}{{\bf local}}
\newcommand{\Hidden}{{\bf hidden}}
%\newcommand{\If}{{\bf if}}
\newcommand{\In}{{\bf in}}
\newcommand{\Implies}{{\bf implies}}
\newcommand{\Includes}{{\bf includes}}
\newcommand{\Introduces}{{\bf introduces}}
\newcommand{\Input}{{\bf input}}
\newcommand{\Kind}{{\bf kind}}
\newcommand{\Initially}{{\bf initially}}
\newcommand{\Internal}{{\bf internal}}
\newcommand{\Inv}{{\bf invariant}}
\newcommand{\Mode}{{\bf mode}}
\newcommand{\Od}{{\bf od}}
\newcommand{\Of}{{\bf of}}
\newcommand{\Output}{{\bf output}}
\newcommand{\Partitioned}{{\bf partitioned}}
\newcommand{\Pre}{{\bf pre}}
\newcommand{\Signature}{{\bf signature}}
\newcommand{\Simulation}{{\bf simulation}}
\newcommand{\Sort}{{\bf sort}}
\newcommand{\States}{{\bf states}}
\newcommand{\Tasks}{{\bf tasks}}
\newcommand{\Then}{{\bf then}}
\newcommand{\To}{{\bf to}}
\newcommand{\Trait}{{\bf trait}}
\newcommand{\Traits}{{\bf traits}}
\newcommand{\Transitions}{{\bf transitions}}
\newcommand{\Trajectories}{{\bf trajectories}}
\newcommand{\Tuple}{{\bf tuple}}
\newcommand{\Type}{{\bf type}}
\newcommand{\Union}{{\bf union}}
\newcommand{\Uses}{{\bf uses}}
\newcommand{\Var}{{\bf variables}}
\newcommand{\Where}{{\bf where}}
%\newcommand{\While}{{\bf while}}
\newcommand{\With}{{\bf with}}


% Spacing
\newcommand{\FFF}{\vspace{0.1in}}
\newcommand{\BBB}{\hspace{-0.1in}}


\newcommand{\deq}{\mathrel{\stackrel{\scriptscriptstyle\Delta}{=}}}


% systematic labels

\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\chapreftwo}[2]{Chapters~\ref{chap:#1}~and~\ref{chap:#2}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\sseclabel}[1]{\label{subsec:#1}}
\newcommand{\ssecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\secreftwo}[2]{Sections~\ref{sec:#1}~and~\ref{sec:#2}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figrefs}[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\lnlabel}[1]{\label{line:#1}}
\newcommand{\lnrngref}[2]{lines~\ref{line:#1}--\ref{line:#2}\xspace}
\newcommand{\lnref}[1]{line~\ref{line:#1}\xspace}
\newcommand{\lemlabel}[1]{\label{lemma:#1}} 
\newcommand{\lemref}[1]{Lemma~\ref{lemma:#1}\xspace}
\newcommand{\thmlabel}[1]{\label{thm:#1}} 
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
\newcommand{\invlabel}[1]{\label{inv:#1}} 
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}\xspace}
\newcommand{\problemlabel}[1]{\label{problem:#1}} 
\newcommand{\problemref}[1]{Problem~\ref{problem:#1}\xspace}
\newcommand{\deflabel}[1]{\label{def:#1}} 
\newcommand{\defref}[1]{Definition~\ref{def:#1}\xspace}
\newcommand{\exerciselabel}[1]{\label{exer:#1}} 
\newcommand{\exerciseref}[1]{Exercise~\ref{exer:#1}\xspace}
\newcommand{\proplabel}[1]{\label{prop:#1}} 
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}\xspace}

% defs FROM ptioa PAPER


\newcommand{\remove}[1]{}
\newcommand{\salg}[1]{\relax\ifmmode {\mathcal F}_{#1}\else ${\mathcal F}_{#1}$\fi} 
\newcommand{\msp}[1]{\relax\ifmmode (#1, \salg{#1}) \else $(#1, \salg{#1})$\fi} 
\newcommand{\msprod}[2]{\relax\ifmmode ( #1 \times #2, \salg{#1} \otimes \salg{#2}) \else $(#1 \times #2, \salg{#1} \otimes \salg{#2})$\fi} 
\newcommand{\dist}[1]{\relax\ifmmode {\mathcal P}\msp{#1}
  \else ${\mathcal P}\msp{#1}$\fi} 
\newcommand{\subdist}[1]{\relax\ifmmode {\mathcal S}{\mathcal P}\msp{#1} 
  \else ${\mathcal S}{\mathcal P}\msp{#1}$\fi} 
\newcommand{\disc}[1]{\relax\ifmmode {\sf Disc}(#1)
  \else ${\sf Disc}(#1)$\fi} 

\newcommand{\Trajeq}{\relax\ifmmode {\mathcal R}_\T \else ${\mathcal R}_\T$\fi} 
\newcommand{\Acteq}{\relax\ifmmode {\mathcal R}_A \else ${\mathcal R}_A$\fi} 
\newcommand{\noop}{\relax\ifmmode \lambda \else $\lambda$\fi} 
\newcommand{\close}[1]{\relax\ifmmode \overline{#1} \else $\overline{#1}$\fi} 

\newcommand{\corrtasks}{\mathop{\mathsf {c}}}
\newcommand{\full}{\mathop{\mathsf {full}}}
%\newcommand{\fstate}{\mathop{\mathsf {fstate}}}
%\newcommand{\lstate}{\mathop{\mathsf {lstate}}}
\newcommand{\tdist}{\mathop{\mathsf {tdist}}}
\newcommand{\extbeh}{\mathop{\mathsf {extbeh}}}
%\newcommand{\apply}{\mathop{\mathsf {apply}}}
\newcommand{\apply}[2]{\mathop{\mathsf {apply}({#1},{#2})}}
%\newcommand{\applytwo}{\mathop{\mathsf {apply2}}}
\newcommand{\support}{\mathop{\mathsf {supp}}}
\newcommand{\relation}{\mathrel{R}}
\newcommand{\cone}{C}
%\newcommand{\tracef}{\mathord{\mathsf {trace}}}
\newcommand{\flatten}{\mathord{\mathsf {flatten}}}
\newcommand{\discrete}{\mathord{\mathsf {Disc}}}
\newcommand{\lift}[1]{\mathrel{{\mathcal L}(#1)}}
\newcommand{\expansion}[1]{\mathrel{{\mathcal E}(#1)}}
%End of commands added by Roberto on May, 12

%>> Ling, December 2005

\newcommand{\subdisc}{\operatorname{\mathsf {SubDisc}}}
\newcommand{\tran}{\operatorname{\mathsf {tran}}}
%\newcommand{\act}{\operatorname{\mathsf {act}}}

\renewcommand{\execs}{{\operatorname{\mathsf {Execs}}}}
\newcommand{\frags}{{\operatorname{\mathsf {Frags}}}}

\newcommand{\tracefnc}{{\operatorname{\mathsf {trace}}}}
\newcommand{\untimefnc}{{\operatorname{\mathsf {untime}}}}

\newcommand{\finite}{{\operatorname{\mathsf {finite}}}}
\newcommand{\hide}{{\operatorname{\mathsf {hide}}}}

\newcommand{\early}{{\operatorname{\mathsf {Early}}}}
\newcommand{\late}{{\operatorname{\mathsf {Late}}}}
\newcommand{\toss}{{\operatorname{\mathsf {Toss}}}}

\newcommand{\define}{:=}

\newcommand{\pc}{{\operatorname{\mathsf {counter}}}}
\newcommand{\chosen}{{\operatorname{\mathsf {chosen}}}}

\newcommand{\rand}{{\operatorname{\mathsf {random}}}}
\newcommand{\unif}{{\operatorname{\mathsf {unif}}}}

\newcommand{\ie}{i.e.,\xspace}
\newcommand{\Ie}{I.e.,\xspace}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}

% IOA related stuff




\newcommand{\mybox}[3]{
  \framebox[#1][l]
  {
    \parbox{#2}
    {
      #3
    }
  }
}

\newcommand{\two}[4]{
  \parbox{.95\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\twosep}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
   	\vrule width 0.2pt
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\eqntwo}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{$ #3 $}
    \parbox[t]{#2\columnwidth}{$ #4 $}
  }}

\newcommand{\three}[6]{\vspace{1pt} \vfill
        \parbox{\columnwidth}{%
        \parbox[t]{#1\columnwidth}{#4}%
        \parbox[t]{#2\columnwidth}{#5}%
        \parbox[t]{#3\columnwidth}{#6}%
      }}

\newcommand{\tup}[1]
           {
             \relax\ifmmode
             ( #1 )
             \else $($ #1 $)$ \fi
           }

\newcommand{\lit}[1]{ \relax\ifmmode
                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}
                \else {\it #1} \fi }


\newcommand{\figuresize}{\scriptsize}

\newcommand{\equationsize}{\footnotesize}

%\newcommand{\act}[1]{%
%  \relax\ifmmode
%                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}%
%                \else
%                {\sf #1\/}%
%                \fi }


\lstdefinelanguage{ioa}{
  basicstyle=\figuresize,
  keywordstyle=\bf \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={automaton, and, actions,
  	 choose,const,continue, components,
  	 discrete, do,
  	 eff, external,else, elseif, evolve, end,
  	 fi,for, forward, from,
  	 hidden,
  	 in,input,internal,if,invariant, initially, imports,
     let,
	mode,
     or, output, operators, od, of,
     pre,
     return,
     such,satisfies, stop, signature, simulation, 
     trajectories,trajdef, transitions, that,then, type, types, to, tasks,
     variables, vocabulary, 
     when,where, with,while},
  emph={set, seq, tuple, map, array, enumeration, powerset},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }

\lstdefinelanguage{ioaNums}[]{ioa}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{ioaNumsRight}[]{ioa}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\ioa}{\lstinline[language=ioa]}

\lstnewenvironment{IOA}%
  {\lstset{language=IOA}}
  {}

\lstnewenvironment{IOANums}%
  {
  \if@firstcolumn
    \lstset{language=IOA, numbers=left, firstnumber=auto}
  \else
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{IOANumsRight}%
  {
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  }
  {}

%\lstnewenvironment{IOA}%
%  {\lstset{language=ioaLang}
%   \csname lst@SetFirstLabel\endcsname}
%  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\newcommand{\figioa}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=ioaLang]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigioa}[9]{

}

\newcommand{\twofigioa}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=ioaLang]{#7}
    }
    {
      \lstinputlisting[language=ioaLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}



\lstdefinelanguage{ioaLang}{%
  basicstyle=\ttfamily\small,
  keywordstyle=\rmfamily\bfseries\small,
  identifierstyle=\small,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,bounds,by,case,choose,components,const,d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,fire,follow,for,forward,from,hidden,if,in,%
    input,initially,internal,invariant,let, local,model,od,of,output,pre,schedule,signature,so,%
    simulation,states,variables, tasks, stop,tasks,that,then,to,trajdef,trajectory,trajectories,transitions,tuple,type,union,urgent,uses,when,where,while,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        {\\rho}{{$\rho$}}1
        {\\infty}{{$\infty$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1 
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1 
        {=>}{{$\Rightarrow$}}1 
        {->}{{$\rightarrow$}}1 
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2 
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}

\lstdefinelanguage{bigIOALang}{%
  basicstyle=\ttfamily,
  keywordstyle=\rmfamily\bfseries,
  identifierstyle=,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,by,case,choose,components,const,%
    d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,for,forward,from,hidden,if,in%
    input,initially,internal,invariant,mode,local,od,of,output,pre,schedule,signature,so,%
    tasks, simulation,states,stop,tasks,that,then,to,trajdef,trajectories,transitions,tuple,type,union,urgent,uses,when,where,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1 
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1 
        {=>}{{$\Rightarrow$}}1 
        {->}{{$\rightarrow$}}1 
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2 
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}


\lstnewenvironment{BigIOA}%
  {\lstset{language=bigIOALang,basicstyle=\ttfamily}
   \csname lst@SetFirstLabel\endcsname}
  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\lstnewenvironment{SmallIOA}%
  {\lstset{language=ioaLang,basicstyle=\ttfamily\scriptsize}
   \csname lst@SetFirstLabel\endcsname}
  %{\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}
  {\csname lst@SaveFirstLabel\endcsname\noindent}


\newcommand{\true}{\relax\ifmmode \mathit true \else \em true \/\fi}
\newcommand{\false}{\relax\ifmmode \mathit false \else \em false \/\fi}


\newcommand{\Real}{{\operatorname{\texttt{Real}}}}
\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}
\newcommand{\Char}{{\operatorname{\texttt{Char}}}}
\newcommand{\ioaInt}{{\operatorname{\texttt{Int}}}}
\newcommand{\ioaNat}{{\operatorname{\texttt{Nat}}}}
\newcommand{\ioaAugR}{{\operatorname{\texttt{AugmentedReal}}}}
\newcommand{\ioaString}{{\operatorname{\texttt{String}}}}
\newcommand{\Discrete}{{\operatorname{\texttt{Discrete}}}}
%\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}

%\newcommand{\lnot}{\neg}
%\newcommand{\land}{\wedge}
%\newcommand{\lor}{\vee}
\newcommand{\limplies}{\Rightarrow}
\newcommand{\liff}{\Leftrightarrow}

\newlength{\bracklen}
\newcommand{\sem}[1]{\settowidth{\bracklen}{[}
     [\hspace{-0.5\bracklen}[#1]\hspace{-0.5\bracklen}]}

\newcommand{\defaultArraystretch}{1.4}
\renewcommand{\arraystretch}{\defaultArraystretch}

\newcommand{\gS}{\mathcal{S}}
\newcommand{\gV}{\mathcal{V}}
\newcommand{\freevars}{\mathcal{FV}}

\newcommand{\gVspec}{\mathcal{V}_\mathit{spec}}
\newcommand{\gVa}{\mathcal{V}_\mathit{A}}
\newcommand{\gVsig}{\mathcal{V}_\mathit{sigs}}
\newcommand{\gVso}{\mathcal{V}_\mathit{sorts}}
\newcommand{\gVop}{\mathcal{V}_\mathit{ops}}
\newcommand{\sort}{\mathit{sort}}
\newcommand{\sig}{\mathit{sig}}
\newcommand{\id}{\mathit{id}}
\newcommand{\sigsep}{\lsl`->`}

%\newcommand{\T}{\mathit{true}}
%\newcommand{\F}{\mathit{false}}

\newcommand{\super}[2]{\ensuremath{\mathit{#1}^\mathit{#2}}}
\newcommand{\tri}[3]{\ensuremath{\mathit{#1}^\mathit{#2}_\mathit{#3}}}
\newcommand{\Assumptions}{\ensuremath{\mathit{Assumptions}}}
\newcommand{\actPred}[3][\pi]{\tri{P}{#2,#1}{#3}}
\newcommand{\actualTypes}[1]{\super{actualTypes}{#1}}
\newcommand{\actuals}[1]{\super{actuals}{#1}}
\newcommand{\autActVars}[2][\pi]{\vars{#2}{},\vars{#2,#1}{}}
\newcommand{\bracket}[2]{\mathit{#1}[\mathit{#2}]}
\newcommand{\compVars}[1]{\super{compVars}{#1}}
\newcommand{\context}{\mathit{context}}
\newcommand{\ensuring}[2]{\tri{ensuring}{#1}{#2}}
\newcommand{\initPred}[1]{\tri{P}{#1}{init}}
\newcommand{\initVals}[1]{\super{initVals}{#1}}
\newcommand{\initially}[2]{\tri{initially}{#1}{#2}}
\newcommand{\invPred}[2]{\tri{Inv}{#1}{#2}}
\newcommand{\knownVars}[1]{\super{knownVars}{#1}}
\newcommand{\localPostVars}[2]{\tri{localPostVars}{#1}{#2}}
\newcommand{\localVars}[2]{\tri{localVars}{#1}{#2}}
\newcommand{\locals}[1]{\bracket{Locals}{#1}}
\newcommand{\nam}[1]{\rho^{\mathit{#1}}}
\newcommand{\otherActPred}[3][\pi]{\otherTri{P}{#2,#1}{#3}}
\newcommand{\otherParams}[2]{\otherTri{params}{#1}{#2}}
\newcommand{\otherSub}[2]{\otherTri{\sigma}{#1}{#2}}
\newcommand{\otherTri}[3]{\tri{\smash{#1'}}{#2}{#3}}
\newcommand{\otherVars}[2]{\otherTri{vars}{#1}{#2}}
\newcommand{\params}[2]{\tri{params}{#1}{#2}}
\newcommand{\postVars}[1]{\super{postVars}{#1}}
\newcommand{\pre}[2]{\tri{Pre}{#1}{#2}}
\newcommand{\prog}[2]{\tri{Prog}{#1}{#2}}
\newcommand{\prov}[2]{\tri{Prov}{#1}{#2}}
\newcommand{\stateSorts}[1]{\super{stateSorts}{#1}}
\newcommand{\stateVars}[1]{\super{stateVars}{#1}}
\newcommand{\states}[1]{\bracket{States}{#1}}
\newcommand{\sub}[2]{\tri{\sigma}{#1}{#2}}
\newcommand{\sugActPred}[3][\pi]{\tri{P}{#2,#1}{#3,desug}}
\newcommand{\sugLocalVars}[2]{\ifthenelse{\equal{}{#2}}%
                             {\tri{localVars}{#1}{desug}}%
                             {\tri{localVars}{#1}{#2,desug}}}
\newcommand{\sugVars}[2]{\ifthenelse{\equal{}{#2}}%
                        {\tri{vars}{#1}{desug}}%
                        {\tri{vars}{#1}{#2,desug}}}
\newcommand{\cVars}[1]{\super{cVars}{#1}}

\newcommand{\vmap}{\dot{\varrho}}
\newcommand{\map}[2]{\tri{\vmap}{#1}{#2}}

\newcommand{\types}[1]{\super{types}{#1}}
\newcommand{\vars}[2]{\tri{vars}{#1}{#2}}

\newcommand{\subActPred}[3][\pi]{\sub{#2,#1}{#3}(\tri{P}{#2,#1}{#3,desug})}
\newcommand{\subLocalVars}[2]{\sub{#1}{#2}(\tri{localVars}{#1}{#2,desug})}

\newcommand{\dA}{\hat{A}}
\newcommand{\renameAction}[1]{\ensuremath{\rho_{#1}(\vars{\dA{#1},\pi}{})}}
\newcommand{\renameComponent}[1]{\ensuremath{\rho_{#1}\dA_{#1}}}

\newenvironment{Syntax}{\[\begin{subSyntax}}{\end{subSyntax}\]\vspace{-.3in}}
\newenvironment{subSyntax}{\begin{array}{l}}{\end{array}}
\newcommand{\w}[1]{\mbox{\hspace*{#1em}}}



%TIOA macros
% Script math symbol name
\newcommand{\ms}[1]{\ifmmode%
\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}\else%
$\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}$\fi}

%\newcommand{\domain}[1]{{\it dom}(#1)} % domain

% KEYWORDS 
\newcommand{\kw}[1]{{\bf #1}} 
\newcommand{\tcon}[1]{{\tt #1}} 
\newcommand{\syn}[1]{{\tt #1}} 
\newcommand{\pvskw}[1]{{\sc #1}} 
\newcommand{\pvsid}[1]{{\operatorname{\mathit{#1}}}}


% VALUATIONS
\newcommand{\vv}{{\bf v}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\va}{{\bf a}}
\newcommand{\vb}{{\bf b}}
\newcommand{\vg}{\mathit{g}}
\newcommand{\vq}{{\bf q}}
\newcommand{\vs}{{\bf s}}
\newcommand{\vm}{{\bf m}}

% Transitions and trajectory operations
\newcommand{\arrow}[1]{\mathrel{\stackrel{#1}{\rightarrow}}}
\newcommand{\sarrow}[2]{\mathrel{\stackrel{#1}{\rightarrow_{#2}}}}
\newcommand{\concat}{\mathbin{^{\frown}}} % concatenation
\newcommand{\paste}{\mathrel{\diamond}}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\groupop}{\circ}

\def\CC{{\mathscr C}} % concatenation closure

% PVS STUFF

\lstdefinelanguage{pvs}{
  basicstyle=\tt \figuresize,
  keywordstyle=\sc \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and, 
  	 begin,
  	 cases, const,
  	 do,
  	 external, else, exists, end, endcases, endif,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure, 
     not,
     or, of,
     return, recursive,
     stop, 
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, enumeration, bool, real, exp, nnreal, posreal},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }



\lstdefinelanguage{BigPVS}{
  basicstyle=\tt,
  keywordstyle=\sc,
  identifierstyle=\it,
  emphstyle=\tt ,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and, 
  	 begin,
  	 cases, const,
  	 do, datatype,
  	 external, else, exists, end, endif, endcases,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure,
     not,
     or, of,
     return, recursive,
     stop, 
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, first, rest, add, enumeration, bool, real, posreal, nnreal},   
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3        
      }

\lstdefinelanguage{pvsNums}[]{pvs}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{pvsNumsRight}[]{pvs}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\pvs}{\lstinline[language=PVS]}

\lstnewenvironment{BigPVS}%
  {\lstset{language=BigPVS}}
  {}

\lstnewenvironment{PVSNums}%
  {
  \if@firstcolumn
    \lstset{language=pvs, numbers=left, firstnumber=auto}
  \else
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{PVSNumsRight}%
  {
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  }
  {}


\newcommand{\figpvs}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=pvs]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigpvs}[9]{

}

\newcommand{\twofigpvs}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=pvsLang]{#7}
    }
    {
      \lstinputlisting[language=pvsLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}


\lstdefinelanguage{pvsproof}{
  basicstyle=\tt \figuresize,
  mathescape=true,
  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
  basewidth=0.05em,
}


\lstdefinelanguage{pseudocode}{
%	basicstyle=\figuresize,
%	keywordstyle=\bf \figuresize,
%	identifierstyle=\it \figuresize,
%	emphstyle=\tt \figuresize,
	mathescape=true,
	tabsize=20,
	xleftmargin=4.0ex,
	basicstyle=\normalsize,
	sensitive=false,
	columns=fullflexible,
	keepspaces=false,
	%flexiblecolumns=true,
	%  basewidth=0.5em,
	basewidth=0.05em,
	moredelim=[il][\rm]{//},
	moredelim=[is][\sf \figuresize]{!}{!},
	moredelim=[is][\bf \figuresize]{*}{*},
	keywords={automaton, algorithm, and, 
		choose,const,continue, components,
		discrete, do,
		eff, external,else, elseif, evolve, end, each, exit,
		fi,for, forward, from, find, 
		hidden,
		in,input,internal,if,invariant, initially, imports,
		let,
		mode,
		or, output, operators, od, of,
		pre,
		return,
		such,satisfies, stop, signature, simulation, sample,
		trajectories,trajdef, transitions, that,then, type, types, to, tasks,
		variables, vocabulary, 
		when,where, with,while},
	emph={set, seq, tuple, map, array, enumeration},   
	literate=
	{(}{{$($}}1
	{)}{{$)$}}1
	% LaTeX math symbols
	{\\in}{{$\in\ $}}1
	{\\preceq}{{$\preceq\ $}}1
	{\\subset}{{$\subset\ $}}1
	{\\subseteq}{{$\subseteq\ $}}1
	{\\supset}{{$\supset\ $}}1
	{\\supseteq}{{$\supseteq\ $}}1
	{\\forall}{{$\forall$}}1
	{\\le}{{$\le\ $}}1
	{\\ge}{{$\ge\ $}}1
	{\\gets}{{$\gets\ $}}1
	{\\cup}{{$\cup\ $}}1
	{\\cap}{{$\cap\ $}}1
	{\\langle}{{$\langle$}}1
	{\\rangle}{{$\rangle$}}1
	{\\exists}{{$\exists\ $}}1
	{\\bot}{{$\bot$}}1
	{\\rip}{{$\rip$}}1
	{\\emptyset}{{$\emptyset$}}1
	{\\notin}{{$\notin\ $}}1
	{\\not\\exists}{{$\not\exists\ $}}1
	{\\ne}{{$\ne\ $}}1
	{\\to}{{$\to\ $}}1
	{\\implies}{{$\implies\ $}}1
	% LSL symbols (one-character)
	{<}{{$<\ $}}1
	{>}{{$>\ $}}1
	{=}{{$=\ $}}1
	{~}{{$\neg\ $}}1
	{|}{{$\mid$}}1
	{'}{{$^\prime$}}1
	% LSL symbols (two characters)
	{\\A}{{$\forall\ $}}1
	{\\E}{{$\exists\ $}}1
	{\\/}{{$\vee\,$}}1
	{\\vee}{{$\vee\,$}}1
	{/\\}{{$\wedge\,$}}1
	{\\wedge}{{$\wedge\,$}}1
	{=>}{{$\Rightarrow\ $}}1
	{->}{{$\rightarrow\ $}}1
	{<=}{{$\Leftarrow\ $}}1
	{<-}{{$\leftarrow\ $}}1
	%        {<=}{{$\leq$}}1
	%        {>=}{{$\geq$}}1
	{~=}{{$\neq\ $}}1
	{\\U}{{$\cup\ $}}1
	{\\I}{{$\cap\ $}}1
	{|-}{{$\vdash\ $}}1
	{-|}{{$\dashv\ $}}1
	{<<}{{$\ll\ $}}2
	{>>}{{$\gg\ $}}2
	{||}{{$\|$}}1
	%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
	%%        {[}{{$\langle$}}1
	%%        {]}{{$\rangle$}}1
	{[}{{$[$}}1
	{]}{{$\,]$}}1
	{[[}{{$\langle$}}1
	{]]]}{{$]\rangle$}}1
	{]]}{{$\rangle$}}1
	{<=>}{{$\Leftrightarrow\ $}}2
	{<->}{{$\leftrightarrow\ $}}2
	{(+)}{{$\oplus\ $}}1
	{(-)}{{$\ominus\ $}}1
	{_i}{{$_{i}$}}1
	{_j}{{$_{j}$}}1
	{_{i,j}}{{$_{i,j}$}}3
	{_{j,i}}{{$_{j,i}$}}3
	{_0}{{$_0$}}1
	{_1}{{$_1$}}1
	{_2}{{$_2$}}1
	{_n}{{$_n$}}1
	{_p}{{$_p$}}1
	{_k}{{$_n$}}1
	{-}{{$\ms{-}$}}1
	{@}{{}}0
	{\\delta}{{$\delta$}}1
	{\\R}{{$\R$}}1
	{\\Rplus}{{$\Rplus$}}1
	{\\N}{{$\N$}}1
	{\\times}{{$\times\ $}}1
	{\\tau}{{$\tau$}}1
	{\\alpha}{{$\alpha$}}1
	{\\beta}{{$\beta$}}1
	{\\gamma}{{$\gamma$}}1
	{\\ell}{{$\ell\ $}}1
%	{--}{{$-\ $}}1
	{\\TT}{{\hspace{1.5em}}}3        
}

\lstdefinelanguage{pseudocodeNums}[]{pseudocode}
{
	numbers=left,
	numberstyle=\tiny,
	stepnumber=2,
	numbersep=4pt
	%  firstnumber=1
}

%%%%%%% Mahesh's macros
%
% Turing machine related macros
%
\newcommand{\blank} {\sqcup} %Blank symbol
\newcommand{\leftendmarker} {\rhd} %Left end marker of TM tape
\newcommand{\lft} {\mathsf{L}} %Left direction
\newcommand{\rght} {\mathsf{R}} %Right direction
\newcommand{\qacc} {q_{\mathsf{acc}}} %Accepting state
\newcommand{\qrej} {q_{\mathsf{rej}}} %Rejecting state
\newcommand{\movetm} {\vdash} %Single move of TM
\newcommand{\movetmst} {{\movetm}^*} %Zero or more moves of TM
\newcommand{\tmcode}[1] {\langle #1 \rangle} %Code of a TM

%%% Simulation driven verification related macros
\newcommand{\interval}{\mathit{interval}} %Code of a TM
\newcommand{\ct}{\mathit{center}} %Code of a TM
\newcommand{\rg}{\mathit{range}} %Code of a TM
\newcommand{\vertex} {\mathit{vertex}} %Code of a TM
\newcommand{\dur}{\mathit{dur}} %Code of a TM
\newcommand{\traj}{\mathit{Traj}} %Code of a TM
\newcommand{\Reach}{\mathit{Reach}} %Code of a TM
\newcommand{\gammahat}{\hat{\gamma}} %Code of a TM
\newcommand{\ldfmnorm}{\mathit{ldfnorm}} %Code of a TM
\newcommand{\Loc}{\mathit{Loc}} %Code of a TM
\newcommand{\Vertex}{{\bf V}} %Code of a TM
\newcommand{\Edge}{{\bf E}} %Code of a TM
\newcommand{\elab}{\mathit{elab}} %Code of a TM
\newcommand{\loc}{\mathit{loc}} %Code of a TM
\newcommand{\trajlab}{{\bf TL}} %Code of a TM
\newcommand{\hs}{\mathit{hs}} %Code of a TM
\newcommand{\init}{\mathit{init}} %Code of a TM
\newcommand{\locinit}{\mathit{locinit}} %Code of a TM
\newcommand{\invariant}{\mathit{invariant}} %Code of a TM
\newcommand{\linit}{\mathit{linit}} %Code of a TM
\newcommand{\Lmode}{\mathit{Lmode}} %Code of a TM
\newcommand{\Execs}{\mathit{Execs}} %Code of a TM
\newcommand{\nextInit}{\mathit{nextInit}} %Code of a TM
\newcommand{\remainTime}{\mathit{tRemain}} %Code of a TM
\newcommand{\simulator}{\mathit{sim}} %Code of a TM
\newcommand{\TB}{\mathit{reachtube}} %safe-reachtube output
\newcommand{\findldf}{\sf{compLDF}} 
\newcommand{\coverstack}{\mathit{coverstack}} 
\newcommand{\Rtube}{\mathit{Rtube}} 
\newcommand{\unsafe}{\bf{U}} %Unsafe set
\newcommand{\intA}{\bf{IntA}} %Interval matrix A
\newcommand{\argmin}[1]{\sf{argmin}_{#1}} %Unsafe set
\newcommand{\InitialQueue}{\mathit{queue}} %initial queue
\newcommand{\reachHybrid}{\mathit{reachtube}} %initial queue

\newcommand{\cachTree}{\mathit{cachetree}}
\newcommand{\rootnode}{\mathit{root}} 
\newcommand{\traversalstack}{\mathit{traversalQueue}} 
\newcommand{\node}{\mathit{node}}
\newcommand{\nodechildren}{\mathit{children}}
\newcommand{\initialset}{\mathit{initset}}
\newcommand{\reachset}{\mathit{Reach}} 
\newcommand{\originalalgo}{\mathit{original}}
\newcommand{\supportalgo}{\mathit{support}}  
\newcommand{\overrt}{\mathit{rt}}

==> sayan-prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

==> sim_driven_verif.tex <==
\subsection{Data-driven verification}
\label{sec:simVerif}
Data-driven verification algorithms  answer the bounded safety verification question using numerical simulation data, that is, samples of the solution $\xi(x_0,t)$.  The key idea is to generalize an individual simulation $\xi(x_0,\cdot)$ to over-approximate the reachtube $\Rtube(B(x_0,\delta),T)$, for some $\delta > 0$. This generalization  covers a $\delta$-ball $B(x_0,\delta)$ of the initial set $K$, and  several simulations can then cover all of $K$ and over-approximate $\Rtube(K,T)$, which in turn could prove safety. If the over-approximations turn out to be too conservative and safety cannot be concluded, then $\delta$ has to be reduced, and more precise over-approximations of $\Rtube(K,T)$ have to be computed with smaller generalization radius $\delta$ and more simulation data. 

Thus far, the generalization strategy has been entirely based on computing sensitivity of the solution $\xi(x_0, t)$ to the initial condition $x_0$. Algorithms have been developed for computing this sensitivity for linear,  nonlinear, and hybrid dynamical models~\cite{breachAD,FanM15:ATVA,FanQM0D16} as well as for estimating sensitivity from black-box systems~\cite{FanQMV:CAV2017}.  The resulting software tools have been successfully applied to  verify  automotive, aerospace, and medical embedded systems~\cite{FanQM18,HuangFMMK14,Prabhakar2015}.


%make this decision using numerical solutions of the ODE system and  {\em sensitivity-analysis\/} of $f$. For the research reported here, we will use the data-driven verification tool C2E2~\cite{FanQM0D16} developed at Illinois. C2E2 computes precise sensitivity functions (formally  {\em discrepancy functions\/}) based on the system model $f$ using the algorithms in~\cite{FanM15:ATVA}. 

 The precise notion of sensitivity needed for the verification algorithm to have soundness and relative completeness is formalized as {\em discrepancy function\/}~\cite{DMVemsoft2013}. 
\begin{definition}
	\label{def:discrepancy}
A discrepancy function of system~(\ref{eq:goal_ode}) with initial set of states $K \subseteq \mathbb{R}^n$ is a class-$\mathcal{K}$ function in the first argument $\beta: \nnreals \times \nnreals \rightarrow \nnreals$ that satisfies the following conditions:
%\begin{inparaenum}
(1) $\forall \ x, x' \in K, t \geq 0$,  
$\|\xi(x,t) - \xi(x',t)\| \leq \beta(\|x - x'\|,t)$,
(2) $\beta(\|\xi(x,t) -\xi(x',t)\|,t) \rightarrow 0$ as $\|x - x'\| \rightarrow 0$.
%\end{inparaenum}
\end{definition}

The first condition in Definition~\ref{def:discrepancy} says that $\beta$ upper-bounds the distance between two trajectories as a function of the distance between their initial states. The second condition makes the bound shrink as the initial states get closer.% There are several methods to compute a discrepancy function using incremental Lyapunov function \cite{Girard2010}, maximal eigenvalues of the Jacobian matrix~\cite{} 
%Thus, as the radius $\delta$  of the partition of the initial set reduces, the over-approximation given by discrepancy function goes down to zero. 
 
Algorithm~\ref{code:safetyVerifAlgo} without the boxed parts describes data-driven verification for a dynamical system~(\ref{eq:goal_ode}). We refer to this algorithm as  $\simVerif$ in this paper. Given the compact initial set of states $K \subseteq \reals^n$, a time bound $T > 0$, and an unsafe set $U$, $\simVerif$ answers the safety verification question. It initializes a stack called $\coverstack$ with a cover of $K$. Then, it checks the safety from each element in  the cover. For a given $B(x_0,\delta)$ in $\coverstack$, $\simVerif$ simulates~(\ref{eq:goal_ode}) from $x_0$ and bloats to compute an over-approximation of $\Rtube(B(x_0,\delta),T)$. Formally, the set $\mathit{sim} \oplus \beta$ is a Minkowski sum. This can be computed by increasing the radius in each dimension of $\mathit{sim}$ at a time instant $t$ by $\beta(\delta, t)$. The first condition on $\beta$ ensures that this set is indeed an over-approximation of $\Rtube(B(x_0,\delta),T)$.
%
If this over-approximation is disjoint from $U$ then it is safe and is removed from $\coverstack$. If instead, the over-approximation intersects with $U$ then that is inconclusive and  $B(x_0,\delta)$ is partitioned into smaller sets and added to $\coverstack$. The second condition on $\beta$ ensures that this {\em refinement\/} leads to a more precise over-approximation of $B(x_0,\delta)$. 
%
On the other hand, if the simulation hits $U$, that serves as  a counterexample and $\simVerif$  returns unsafe. %it cannot decide if it intersects it because of an actual trajectory starting from $K$ or because of the overapproximation error. 
Finally, if $\coverstack$ becomes empty, that implies that the algorithm reached a partition of $K$ from which all the over-approximated reachtubes are disjoint from $U$, and then $\simVerif$ returns safe.
\begin{algorithm}
	\small
	\caption{$\simVerif$ safety verification algorithm}
		\label{code:safetyVerifAlgo}
%\begin{algorithm}	
	\begin{algorithmic}[1]
		\State \textbf{input:} $K, T, U, \Gamma, \beta$
		\State $\coverstack \gets$ finite cover $ \cup_i B(x_i,\delta) \supseteq K$
		\State \tikzmark{startsym1} $\cachTree \gets \emptyset$ \tikzmark{endsym1} \label{ln:initcahcetree}
		\While{$\coverstack \neq \emptyset$}
		\State $B(x_0,\delta) = \coverstack.pop()$
		%\State $\coverstack \gets \coverstack \textbackslash \{B(x_0,\delta)\}$
		\State \tikzmark{startsym}$ ans \gets {\sf{SymmetryandRefine}}(U,\Gamma, \cachTree,B(x_0,\delta))$ \label{ln:symmetrycall}
		\If{$ans = {\sf{Unsafe}}$} 
		\textbf{return:} $ans$
		\ElsIf{$ ans = {\sf{Safe}}$}
		 \textbf{continue} 
		\Else \tikzmark{endsym}\label{ln:endSymBlock}
		\State $\mathit{sim} \gets $simulate  $\xi(x_0,\cdot)$ upto time $T$ \label{ln:sim}
		\State $rt \gets  \mathit{sim} \oplus \beta$ \label{ln:rt}
		\State \tikzmark{startsym2} $\cachTree.insert(node(rt,sim))$\tikzmark{endsym2} \label{ln:addNodeTree} 
		\If{$\mathit{sim}$ intersects with $U$ } 
		\State \textbf{return:} {\sf{Unsafe}}
		\ElsIf{$rt$ intersects with $U$}
		 \State Refine cover and add to the $\coverstack$
		\EndIf
		\EndIf
		\EndWhile
		\State \textbf{return:} {\sf{Safe}}
	\end{algorithmic}
%
\Textbox{startsym1}{endsym1}{}
\Textbox[6.25cm]{startsym}{endsym}{}
\Textbox{startsym2}{endsym2}{}
\end{algorithm}



%\sayan{What is the difference between $\beta$ and $\gamma$?}



%Soundness and relative completeness.



==> sym_ode.tex <==
\subsection{Symmetry in dynamical systems}
\label{sec:symODE}

Symmetry takes a central place in analysis of dynamical systems~\cite{Marsden:2010:IMS:1965128}. The research line pertinent to our work develops the conditions under which one can get a solution by transforming another solution~\cite{MarsdenRatiu2010,Olver1986,freund_1986}. First, recall the definition of a group.

\begin{definition} A group $(\Gamma,\groupop)$ is a set $\Gamma$ and an operator $\groupop:\Gamma \times \Gamma \rightarrow \Gamma$ satisfying:
\begin{itemize}
\item Closure: For any $\gamma_1, \gamma_2 \in \Gamma$, $\gamma_1 \groupop \gamma_2 \in \Gamma$
\item Associativity: For any $\gamma_1,\gamma_2,\gamma_3 \in \Gamma$, $\gamma_1 \groupop (\gamma_2 \groupop \gamma_3) = (\gamma_1 \groupop \gamma_2 ) \groupop \gamma_3$.
\item Identity: There is an element $e \in \Gamma$ such that $e \groupop \gamma = \gamma \groupop e = \gamma$.
\item Inverse: For every element $\gamma \in \Gamma$, there exists a unique element $\gamma^{-1} \in \Gamma$, called its inverse, such that $\gamma \groupop \gamma^{-1} =  \gamma^{-1} \groupop \gamma = e$.
\end{itemize}
\end{definition}
%\vspace{-.1in}
Symmetries of dynamical systems are modeled as groups of operators on the state space. 
\vspace{-.1in}
%We now define symmetry in dynamical systems.
\begin{definition}[Definition 2 in \cite{russo2011symmetries}]
	\label{def:symmetry}
	Let $\Gamma$ be a group of operators acting on $\mathbb{R}^n$. We say that $\gamma \in \Gamma$ is a symmetry of (\ref{eq:goal_ode}) if for any solution, $\xi(x_0,t)$, $\gamma \cdot \xi(x_0,t)$ is also a solution. Furthermore, if $\gamma \cdot \xi = \xi$, we say that the solution $\xi$ is $\gamma$-symmetric.
\end{definition}
%\vspace{-.1in}
Thus, if $\gamma$ is a symmetry for (\ref{eq:goal_ode}), then new solutions can be obtained by just applying $\gamma$ to existing solutions. Herein lies the opportunity of exploiting symmetries in data-driven verification. 

How can we know that $\gamma$ is a symmetry for (\ref{eq:goal_ode})? 
It turns out that, a sufficient condition exists that  can be checked without finding the solutions (potentially hard problem), but only by checking commutativity of $\gamma$ with the dynamic function $f$. Systems that meet this criterion are called {\em equivariant}. 



\begin{definition} [Definition 3 in \cite{russo2011symmetries}]
	\label{def:equivariance}
	Let $\Gamma$ be a group of operators acting on $\reals^n$. The dynamic function (vector field) $f: \reals^n \rightarrow \reals^n$  is said to be {\em $\Gamma$-equivariant\/} if $f(\gamma (x)) = \gamma (f(x))$, for any $\gamma \in \Gamma$ and $x \in \reals^n$.
\end{definition}

The following theorem shows that for equivariant systems, solutions are symmetric. 
\begin{theorem}[\cite{golubitsky2012symmetry,russo2011symmetries}]
	\label{thm:sol_transform}
	If~(\ref{eq:goal_ode}) is $\Gamma$-equivariant and $\xi$ is a solution, then so is $\gamma \cdot \xi$, $\forall \gamma \in \Gamma$.
\end{theorem}
\vspace{-.2in}
\section{Symmetries in cyber-physical systems}
\label{sec:symmetry:cps}
\vspace{-.1in}
 Equivariant systems are ubiquitous in nature and in relevant models of cyber-physical systems. Below are few examples of simple equivariant systems with respect to different symmetries. We start with a simple 2-dimensional linear system.

%\sayan{Can we make this a little more interesting? Maybe a diagonal system? scaling + translation together? Why starting with Example 2?}
\begin{example}
	Consider the system 
	\begin{align}
	\label{eq:simplelinear}
	\dot{x}_1 = - x_2, \dot{x}_2 = x_1.
	\end{align}
	where $x_1, x_2 \in \mathbb{R}$.
	Let $\Gamma$ be the set of matrices of the form: 
	$B = [[a,-b], [b,a]]$
	where $a, b \in \mathbb{R}$ and $B$ is not the zero matrix. 
	 Let $\groupop$ be the matrix multiplication operator, then system~(\ref{eq:simplelinear}) is $\Gamma$-equivariant.
	
\end{example}

\begin{example}
Lorenz attractor models the two-dimensional motion of a fluid in a container. Its dynamics are as follows:
\begin{align}
\label{eq:lorenz}
\dot{x} = -px + py, \dot{y} = -xz + rx - y, \dot{z} = xy - bz. 
\end{align}
where $p,r,$ and $b$ are parameters and $x,y$ and $z \in \mathbb{R}$.
Let $\Gamma$ be the group that contains $\gamma: (x,y,z) \rightarrow (-x,-y,z)$ and the identity map. Then, system~(\ref{eq:lorenz}) is $\Gamma$-equivariant\footnote{\url{http://www.scholarpedia.org/article/Equivariant_dynamical_systems}}.
\end{example}

\begin{example}
	\label{eg:car_trans}
	%\sayan{This is the unicycle model I think. Dubins model has a turning radius/length.}
Third, a car model is equivariant to the group of all translations of its position. The car model is described with the following ODEs:
\begin{align}
\label{eq:dubin}
\dot{x} = v \cos \theta, \dot{y} = v \sin \theta, \dot{\phi} = u, \dot{v} = a, \dot{\theta} = \frac{v}{L} \tan(\phi). 
\end{align}
where $u$ and $a$ can be any control signals and $x, y, v, \theta, $and $ \phi \in \mathbb{R}$. We denote $r = (x,y,v,\phi,\theta) = (p,\bar{p})$, where $p = (x,y)$. Let $\Gamma$ be the set of translations of the form $\gamma: r = (p,\bar{p})\rightarrow r' = (p + c,\bar{p})$, for all $c \in \mathbb{R}^2$. 
%Let it also consists of the maps $(x,y,\theta)\rightarrow (-x,-y,\theta +\pi)$, $(x,y,\theta)\rightarrow (-y,x,\theta +\pi/2)$ and $(x,y,\theta)\rightarrow (x,y,\pi/2)$. 
Then, system~(\ref{eq:dubin}) is $\Gamma$-equivariant.
\end{example} 

\begin{example}
	\label{ex:perm_cars}
	Consider the system of two cars with states $r_1$ and $r_2$. Let $\Gamma$ be the set containing the operator $\gamma: (r_1,r_2) \rightarrow (r_2,r_1)$ and the identity operator. Moreover, assume that $u$ and $a$ are the same for both cars. Then, the system is $\Gamma$-equivariant. 
\end{example}
\begin{example}
	
	Let $\Gamma$ be the group generated by the set of transformations of the form $\gamma: (r_1,r_2) = ((p_1,\bar{p}_1), (p_2,\bar{p}_2)) \rightarrow (r_1',r_2') = ((p_1 + c_1,\bar{p}_1), (p_2 + c_2,\bar{p}_2))$, where $c_1$ and $c_2 \in \mathbb{R}^2$, along with the group described in example~\ref{ex:perm_cars}. Then, the system is $\Gamma$-equivariant. Hence, the system is equivariant to translations in the positions of both cars. 
\end{example}

%\sayan{End with a complex example with multiple cars with interesting road geometry. Show informally permutation, together with translation, and rotation. }

%\begin{definition}
%	The set $\Gamma \cdot \xi(t)= \{ \gamma \cdot \xi(t) | \gamma \in \Gamma \}$ is called the group orbit of $\xi(t)$; thus, if we find one solution to an equivariant ordinary differential equation, the whole group orbit of this solution will also exist as solutions.
%\end{definition}


%Definitions.

%Examples.

%Well-known results for moving solutions.
% Should we put the result here?

\begin{comment}
\subsection{Types of Symmetry}
\label{sec:types}
In this section, we discuss the different types of symmetry operators that we consider in this paper, particularly in the experiments.


\paragraph{Linear Transformations for Linear Systems:} Assume that system~(\ref{eq:goal_ode}) is a linear system, i.e. $f(x) = A x$ for some $A \in \mathbb{R}^{n \times n}$ and for all $x \in \mathbb{R}^n$. Let $\Gamma$ be the group of linear operators acting on $\mathbb{R}^n$ that are invertible and commute with $A$, i.e. operators of the form $\gamma(x) = B x$, for all $x \in \mathbb{R}^n$ and for some $B \in \mathbb{R}^{n\times n}$,  where $AB = BA$ and $B^{-1}$ exists. Then, system~(\ref{eq:goal_ode}) is $\Gamma$-equivariant.
The correctness of this claim follows from the condition in Definition~\ref{def:equivariance} on the commutativity of $f$ and $\gamma$.

\paragraph{Permutations:} The third type of symmetry we consider is permutation. In systems with multiple agents such as platoons of cars or coupled oscillators, the identity of each agent does not matter in the evolution of the system. Hence, the system is equivariant to the group of permutations of the variables of the different agents in the state of the system. 

\paragraph{Limited Translations:} Some systems are equivariant for specific group of translation operators (translation vectors). For example, systems with trigonometric-based nonlinearities may be equivariant to fixed translation vectors in the angles in the state because of trigonometric identities.  


\paragraph{Arbitrary Translations:} Assume that a subset $D \subseteq [n]$ does not appear on the right-hand side of the differential equation, i.e. $f(x) = f(x')$ for all $x, x' \in \mathbb{R}^n$ such that $x_i = x_i'$ for all $i \in [n] \textbackslash D$. Moreover, let $\Gamma$ be the group of all operators that change the values of the components with indices in $D$. Then, $f$ is $\Gamma$-equivariant. This type of symmetry is common in kinematic models where the absolute position of the agent does not affect the dynamics.



These groups of operators are simple and are a first step toward a wider use of symmetry in safety verification of hybrid systems.


%This is where we develop the different types of symmetries for linear and nonlinear systems. Could be a long list of examples, or definitions. 
\end{comment}


==> sym_reachsets.tex <==


\section{Symmetry for verification}
\label{sec:reachset_transform}
In this section, we present new results that use symmetry ideas of Section~\ref{sec:symODE} towards  safety verification. We show how symmetry operators can be used to get new reachtubes by transforming existing ones.  This is important for data-driven verification because computation of new reachtubes is in general more expensive than transforming ones. We derived similar theorems for switched systems in Appendix~\ref{sec:app_switched_systems}.
%s can be much more efficient. 
%Then, in Section~\ref{sec:types}, we list the types of symmetries that we consider in the paper. 
%\subsection{Symmetry Transformations for Reachsets}
%\label{sec:reachset_transform}
%In this section, we will be describing how symmetry can be used in reachability-based safety verification. We will show, based on the literature described in Section~\ref{sec:symODE}, that 
%we can transform an already computed reachtube of the system starting from a set of states to get another one that starts from a different set of states. 
For convenience, we will fix a set of initial states $K \subseteq \reals^n$, a time bound $T>0$, a group $\Gamma$ of operators on $\reals^n$, and an operator $\gamma \in \Gamma$ throughout this section. 

The following theorem formalizes transformation of reachtubes based on symmetry. It follows from Theorem~\ref{thm:sol_transform} and the proof can be found in Appendix~\ref{sec:app_reachtube_transform_proof}.
\vspace{-0.02in}
\begin{restatable}[]{theorem}{thmreachtubetransform}
	\label{thm:reachtube_transform}
If (\ref{eq:goal_ode}) is $\Gamma$-equivariant, then $\forall \gamma \in \Gamma$, 
 $\gamma(\Rtube(K,T)) = \Rtube(\gamma (K),T)$.
\end{restatable}
\vspace{-0.02in}
\begin{comment}
\sayan{I made the theorem statement more succinct, see if you agree. Earlier you had words ``reach tube from .. of duration .. T. We have a nice notation for that, why not use it? Rewrite the proof in more detail. At least show $\gamma(\Rtube(K,T)) \subseteq \Rtube(\gamma (K),T)$ and 
$ \Rtube(\gamma (K),T) \subseteq \gamma(\Rtube(K,T)) $.}
\begin{proof} (Sketch)
By Theorem~\ref{thm:sol_transform}, given any solution $\xi(x_0,\cdot)$ of system~(\ref{eq:goal_ode}), where $x_0 \in K$, $\gamma \groupop \xi(x_0, \cdot)$ is its solution starting from $\gamma(x_0)$. Since $\Rtube(K,T)$ is a representation of the set of trajectories starting from $K$ and running for $T$ seconds, these trajectories get transformed to trajectories starting from $\gamma(K)$, and $\gamma ( \Rtube(K,T))$ is the transformation of every state in $\Rtube(K,T)$ at every time step under $\gamma$, then $\gamma (\Rtube(K,T))$ is the reachtube of system~(\ref{eq:goal_ode}) starting from $\gamma (K)$ and running for $T$ seconds. 
\end{proof}
\end{comment}


Corollary~\ref{cor:reachtube_transform} shows how a new reachtube from a set of initial states $K' \subseteq \reals^n$ can be computed by $\gamma$-transforming an existing $\Reach(K,T)$.
%\vspace{-0.02in}
\begin{restatable}[]{corollary}{correachtubetransform}
	\label{cor:reachtube_transform}
If system~(\ref{eq:goal_ode}) is $\Gamma$-equivariant, and $K' \subseteq \mathbb{R}^n$, then if there exists $\gamma \in \Gamma$ such that $K' \subseteq \gamma(K)$, then 
$\Rtube(K',T) \subseteq\gamma(\Rtube(K,T))$.
\end{restatable}
%\vspace{-0.02in}
%We extend the result for switched systems in the following theorem. We fix a switching signal $\sigma$ for the rest of the section. Let $s_0=0, s_1, s_2, \dots s_h =T$ be the switching times in $\sigma$ before and including $T$.  For convenience, we denote by $K_j$ the reachable set of states at exactly the $j^{\mathit{th}}$ switch starting from $K_0 = K$, i.e.  $K_j := \Reach_\sigma(K,s_j)$. In other words, $K_j$ is the initial set of states for the subsystem active after the $j^{\mathit{th}}$ switch. 

%The following remark extend results of this section to reachsets and to the case where we do not have exact reachtubes, but only over-approximations of them. 

\begin{remark}
	\label{rm:over_appr_cor}
Corollary~\ref{cor:reachtube_transform} remains true if instead of $\Rtube(K,T)$, we have a tube that over-approximates it. Moreover,  Theorem~\ref{thm:reachtube_transform} and Corollary~\ref{cor:reachtube_transform}  are also true if we replace the reachtubes with reachsets.
\end{remark}
\vspace{-0.15in}

==> types_of_sym.tex <==
\subsection{Types of Symmetry}
\label{sec:types}
In this section, we discuss the different types of symmetry operators that we consider in this paper, particularly in the experiments.


\paragraph{Linear Transformations for Linear Systems:} Assume that system~(\ref{eq:goal_ode}) is a linear system, i.e. $f(x) = A x$ for some $A \in \mathbb{R}^{n \times n}$ and for all $x \in \mathbb{R}^n$. Let $\Gamma$ be the group of linear operators acting on $\mathbb{R}^n$ that are invertible and commute with $A$, i.e. operators of the form $\gamma(x) = B x$, for all $x \in \mathbb{R}^n$ and for some $B \in \mathbb{R}^{n\times n}$,  where $AB = BA$. Then, (\ref{eq:goal_ode}) is $\Gamma$-equivariant.
The correctness of this claim follows from the condition in Definition~\ref{def:equivariance} on the commutativity of $f$ and $\gamma$.


\paragraph{Arbitrary Translations:} Assume that a subset $S\subseteq [n]$ does not appear on the right-hand side of the differential equation, i.e. $f(x) = f(x')$ for all $x, x' \in \mathbb{R}^n$ such that $x_i = x_i'$ for all $i \in [n] \textbackslash S$. Moreover, let $\Gamma$ be the group of all operators that change the values of the components with indices in $S$. Then, $f$ is $\Gamma$-equivariant. This type of symmetry is common in kinematic models where the absolute position of the agent does not affect the dynamics.

\paragraph{Permutations:} The third type of symmetry we consider is permutation. In systems with multiple agents such as platoons of cars or coupled oscillators, the identity of each agent does not matter in the evolution of the system. Hence, the system is equivariant to the group of permutations of the variables of the different agents in the state of the system. 

\paragraph{Limited Translations:} Some systems are equivariant for specific group of translation operators (translation vectors). For example, systems with trigonometric-based nonlinearities may be equivariant to fixed translation vectors in the angles in the state because of trigonometric identities.  

These groups of operators are simple and are a first step toward a wider use of symmetry in safety verification of hybrid systems.


This is where we develop the different types of symmetries for linear and nonlinear systems. Could be a long list of examples, or definitions. 


==> unboundedsafety.tex <==
\section{Unbounded Reachability Algorithm using Virtual system}
\label{sec:unboundedreachability}

In this section, we use the concept of the virtual system $\ha_v$ to verify unbounded safety properties of the real system $\ha$, i.e. we verify the safety of hybrid automatons with paths of infinite lengths. 
The straight forward solution of using $\computereachset$ to compute the reachset of $\ha$ and intersect it with the unsafe set is not a feasible one. The breadth first search would not terminate and the fixed point in (\ref{eq:fixed_point_condition}) may not be reached if the reachset is an unbounded set and new modes are constantly being discovered along the infinite paths. 

From the previous section, we know that we can transform a sequence of reachset segments of $\ha_v$ to get the reachset of $\ha$. Moreover, we know as well from Definition~\ref{def:hybridautomata_virtual} that the corresponding virtual system may have finite number of modes and its reachset may be a bounded set, when the edges and continuous dynamics in $\ha$ are nice per Section~\ref{sec:virtual_system_discussion}. Hence, the chances of reaching a fixed point for the virtual system are higher. If a fixed point has been reached, the output $\permodedict$ of $\computereachset$ can be used as in Corollary~\ref{cor:vir_dict_to_real_reachset}.


we consider a scenario where we have a model $h: P \rightarrow P$ that defines the edges of the real model, i.e. defines the set of waypoints given the previous waypoint, i.e. $p_{i+1} = h(p_{i})$. Such a model can be for example a finite/infinite state machine or discrete time linear or nonlinear dynamical system. We reduce the unbounded safety verification problem of the real system to the following question: 
 
 the virtual model has the initial set and the initial parameter as part of the model.



 

In this section, we will discuss how to get the infinite reachset of the virtual system. This will be, along with the symmetry transformations in $\Gamma_v$, a representation of the reachset of the real system using Theorem~\ref{thm:realset_from_virtualset}. That in turn would be used for the unbounded safety verification of the real system later in Section~\ref{sec:unboundedsafety}.



\begin{example}[Fixed-wing aircraft unbounded time safety]
	\label{sec:unbounded_example}
	Consider a sequence of modes $ p_0 = [0,0,10,0], p_1 = [10,0,10,10]$, $p_3 = [10,10, 0,10]$, $p_4 = [0,10,0,20]$, $p_5 = [0,20,20,20], p_6 = [20,20,20,30] \dots $ in $P$ which draw a vertical concatenations of $S$ shaped paths with segments of size 10. Assume that the aircraft in Example~\ref{sec:single_drone_example} switches between different modes once its position $[\state[2], \state[3]]$ is in the square with side equal to $1$ around the destination waypoint $[p_i[2],p_i[3]]$, the absolute value of the angle with the segment is at most $\frac{\pi}{6}$, and its speed within $0.5$ of $v_c$. We call this the $\mathit{guard}(p_i)$. Moreover, we assume that for each waypoint, there exists a corresponding unsafe set $U_{p_i} = [[0, -\infty, b_1,b_2],[\infty,\infty,u_1,u_2]]$, where the square $[[b_1,b_2],[u_1,u_2]]$ has radius 1 and center 2 units to the left of the center of the segment of $p_i$. One would verify the safety of such a system by computing the reachtube $\rtube_{p_i}$ of a mode $p_i$ and checking if it is safe by intersecting with $U_{p_i}$. If it is safe, we compute the intersection of $\rtube_{p_i}$ with $\mathit{guard}(p_i)$ to get the initial set for $p_{i+1}$, and repeat the process again. However, we know that the initial set of any mode $p_i$ is at most $\mathit{guard}(p_i)$ which we know its relative position with respect to the segment. Moreover, we know the position of the unsafe set with respect to the segment. Then, one can deduce the unbounded-time safety of this system by just checking the safety of one segment as all scenarios are the same in the virtual system.
	
\end{example}

\begin{comment}

\subsection{Fixed point algorithm}



Now, we union all the guard functions corresponding to a parameter $p_v$ and define the new function:
\begin{align}
\guardsingle_v(p_v) := \cup_{p_v' \in P} \guard(p_v,p_v'). 
\end{align}
The set $\guardsingle_v(p_v)$ represent the set of all possible final states when the relative virtual parameter is $p_v$ before switching to any other parameter.

Similar to the guard function, we union all the reset functions corresponding to a parameter $p_v'$ and define the new function:
\begin{align}
\resetsingle_v(p_v') := \cup_{p_v \in P} \reset(p_v,p_v'). 
\end{align}
The set $\resetsingle(p_v')$ represent the set of all possible initial states when the relative virtual parameter is $p_v'$.


Suppose $G$ is such that $G \circ G$ is defined.  Let $v_{\mathit{term}}$ be the unique terminal  vertex  of $G$.   For  natural  number $i \geq 1$,  define $H_i = \langle L,\theta,G^i,TL \rangle$, where $G^i$ is  the $i$-fold  sequential  composition  of $G$ with  itself.   In  particular, $H_1= \langle L,\theta,G,TL \rangle$.  If $\mathtt{Reach}_{\mathcal{H}_1}^{v_{\mathit{term}}} \subseteq \theta$ then for all $i$, $\mathtt{Reach}_{\mathcal{H}_i} \subseteq \mathtt{Reach}_{\mathcal{H}_1}$. Let $\Gamma$ be a group of symmetry transformations of the system and that all modes have the same dynamics but potentially different guards. If $\exists\ \Gamma_s \subseteq \Gamma$ such that $\mathtt{Reach}_{\mathcal{H}_1}^{v_{\mathit{term}}} \subseteq \cup_{\gamma \in \Gamma_s} \gamma(\theta)$, then $\mathtt{Reach}_{\mathcal{H}_2} \subseteq \cup_{\gamma \in \Gamma_s \cup I} \gamma(\mathtt{Reach}_{\mathcal{H}_1})$. Thus, $\mathtt{Reach}_{\mathcal{H}_i} \subseteq \cup_{j \in [i], \gamma \in \Gamma_s \cup I} \gamma^i(\mathtt{Reach}_{\mathcal{H}_1})$. 



\subsection{Representation}
Hybrid automaton with resets. The waypoints would be changed in the reset. We can model them as continuous variables that we would change in the resets. The guards would be function of these variables.



\subsection{}

Yeah it is time for some concrete theory:


Theorem: Let $p \in P$ be a set of modes,


Consider the state $x$ and the parameters $p$, the virtual parameter $p_v$. 

Consider a hybrid system modeled as a single mode with loop transition. At each transition, $p$ would be updated but $x$ wouldn’t. Instead, it evolves continuously inside each mode. The transition guard is a function of $x$ and $p$. If $\gamma_p(Guard(x, p)) \subseteq  G_v^*$ for all $p \in P_s$, .



\subsection{Infinite S example}
Consider a fixed-wing drone following a path consists of infinite concatenated S shapes. It can be represented as a hybrid automaton with four modes with resets on transitions. The dynamics depends on the current state $x \in \mathbb{R}^4$ and the parameter $p \in \mathbb{R}^2$. The transition of the first mode to the second one updates $p$ by adding 10 to $p[0]$, the second to third mode by adding 5 to $p[1]$, the third to the fourth by subtracting 10 from $p[0]$, and finally the fourth to the first by adding 5 to $p[1]$. The guards on the transitions are a linear function of $x$ and $p$ called $Guard_m(p)$, where $m \in \{1,2,3,4\}$ representing the four modes. Assume that the dynamics has a symmetry transformation $\gamma$ that is a linear function of $x$ and $p$. The transformation of $x$ and $p$ using $\gamma$ is denoted by $\gamma(x,p)$ and is such that $\gamma(x,p) = (x_v, p_v)$. Assume for simplicity  that all modes have the time bound. 

\begin{theorem}[No cache misses]
If the initial set after the $i^{\mathit{th}}$ transition $\initset^i$ and the transformation $\gamma$ have the property that there exists $m \in M$ such that  $\gamma(\initset^i, p_i) \subseteq (\initset_{m}^{v}, p_v)$ and all the modes have the same time bound, then it is enough to compute the reachtube starting from $\initset_m^v$ for all $m \in M$ and that starting from the initial set to make sure that there will be no cache misses.
\end{theorem}

The problem is that $\initset_m^v$s can be very large. So, it would be conservative to compute the reachtubes starting from them. 

\begin{theorem}
Let $Reach_v^i$ be the union of the reachtubes that has been computed so far in the virtual coordinates till the $i^{\mathit{th}}$ transition. If $ \gamma_{p_{i+1}}( Reach_v^i \cap Guard(p_i)) \subseteq \cup\ \initset_v^i$ implies that $Reach_v^{i+1} = Reach_v^{i}$.
\end{theorem}

Let $\Gamma:= \{\gamma : \exists\ i\geq 0, \gamma = \gamma_{p_{i+1}} \gamma_{p_{i}}^{-1} \}$ and $\mathcal{G}_v := \{G_v \subseteq \mathbb{R}^n: \exists \ i\geq 0, G_v = \gamma_{p_i}(Guard(p_i)) \}$.

\begin{corollary}
If $\cup_{\gamma \in \Gamma, G_v \in \mathcal{G}_v}\ \gamma (Reach_v^i \cap G_v) \subseteq \cup\ \initset_v^i$, then we will not have cache misses for unbounded time. 
\end{corollary}


%Define the abstraction map $A: \mathbb{R}^m \times \mathbb{R}^m \rightarrow \mathbb{R}^m \times \mathbb{R}^m$

$\mathcal{D}_v := \{ (p_s, K_v, G_v, \gamma_v): \exists i \geq 0, (p_i, p_{i+1}) \in P^2, p_s = \gamma_{p_{i+1}}(p_i), K_v = \gamma_{p_{i+1}}(Guard(p_i)), G_v = \gamma_{p_{i+1}}(Guard(p_{i+1})), \gamma = \gamma_{p_{i+1}} \gamma_{p_{i}}^{-1} \}$. Let $\mathcal{E}_v := \{(p_s, p_s') \in P^2, \exists i \geq 0, p_s = \gamma_{p_{i+1}}(p_i), p_s' = \gamma_{p_{i+2}}(p_{i+1}) \}$.

\begin{corollary}
If we have the reachtubes starting from all $K_v$s in $\mathcal{D}_v$ computed, then we will not have any cache misses for unbounded time.
\end{corollary} 

Unfortunately, the $K_v$s are large and may be infinite in some dimensions such as the heading angle and the velocity of the fixed aircraft example. The idea is to check what part of $K_v$ would be actually an initial set for some mode $p_i$. This is equivalent to checking to what part of the reachtube intersects the guard. 

Let $Reach^i(p_s)$ be the computed reachtube corresponding to any mode $p_i$ such that $p_s = \gamma_{p_{i+1}}(p_i)$. Then, $Reach_v^i = \cup\ Reach^i(p_s)$. 

\begin{corollary}
If for each $(p_s, p_s') \in \mathcal{E}_v$, $\gamma (Reach^i(p_s) \cap \mathcal{G}_v ) \subseteq Reach^i(p_s').\mathit{initset}$, then we will not have any more cache misses.
\end{corollary}

\begin{corollary}
	Using the previous corollary, we can transform the problem from nonlinear analysis to linear analysis if the updates of the parameters are linear. We can simulate the parameter system disregarding the nonlinear properties of the system, and then bloat every parameter using the corresponding reachtube.
\end{corollary}




\begin{algorithm}
	\small
	% : Symmetry annotation for reachtube computations
	\caption{Unbounded reachability}
	\label{code:unboundednessChecking}
	%\begin{algorithm}	
	\begin{algorithmic}[1]
		\State \textbf{input:} $\{Path_i\}_{i=1}^N, \{K_i\}_{i=1}^N, \Gamma, p_v$
		\State $\mathcal{E} = \emptyset$
		\For{$i \in [N]$}
		\For{$j \in [len(Path_i)-2]$}
		\State $p_j \gets Path_i[j], p_{j+1} \gets Path_i[j+1], p_{j+2} = Path_i[j+2]$
		\State $p_s \gets \gamma_{p_{i+1}}(p_i), p_v \gets \gamma_{p_{i+1}}(p_{i+1}), p_s' \gets \gamma_{p_{i+2}}(p_{i+1})$
		\State $e = (p_s, p_s')$
		\State $\mathcal{E}.add(e)$
		\State $\mathit{Guard}(e) \gets \mathit{Guard}(e)\ \cup\ \gamma_{p_{i+1}}(Guard(p_{i+1}))$
		\EndFor 
		\EndFor
		\For{$i \in [N]$}
		\State $\mathit{tempinitset} \gets K_i$ 
		\For{$j \in [len(Path_i)-2]$}
		\State $p_j \gets Path_i[j], p_{j+1} \gets Path_i[j+1], p_{j+2} = Path_i[j+2]$
		\State $p_s \gets \gamma_{p_{i+1}}(p_i), p_v \gets \gamma_{p_{i+1}}(p_{i+1}), p_s' \gets \gamma_{p_{i+2}}(p_{i+1})$
		\State $e \gets (p_s, p_s')$
		\State $\mathit{initset}(p_s) \gets \mathit{initiset}(p_s)\ \cup\ \mathit{tempinitset}$
		\State $\mathit{tempreach} \gets \mathsf{computeReachtube}(\mathit{tempinitset}, T)$
		\State $\mathit{uncoveredsets}(p_s) \gets \mathit{uncoveredsets}(p_s)\ \textbackslash\ \mathit{tempinitset}$
		\State $\mathit{tempinitset} \gets \cup\  \gamma_{p_{i+2}}(\gamma_{p_{i+1}}^{-1}(\mathit{tempreach} \cap Guard(e)))$
		\State $\mathit{uncoveredsets}(p_s') \gets \mathit{uncoveredsets}(p_s')\ \cup\ (\mathit{tempinitset}\ \textbackslash \mathit{initset}(p_s'))$
		\State $Reach(p_s) \gets Reach(p_s)\ \cup\ \mathit{tempreach}$
		\If{$\forall p_s,\ \mathit{uncoveredsets}(p_s) = \emptyset$}
		\State $\mathbf{return:} $ No more computations are needed
		\EndIf
		\EndFor 
		\EndFor
	\end{algorithmic}
\end{algorithm}


\begin{remark}
	The analysis changed from the state space where the state evolves nonlinearly to the mode space where the mode evolves linear/finite state machine...
\end{remark}



Assume now that the cardinalities of $\Gamma$ and $\mathcal{G}_v$ are finite.

The set of possible mode initial sets in the virtual coordinates is:
  $\mathcal{K}_v = \{ K: K = \gamma_{p_{i+1}}(Guard(p_i))\}$.

The set of possible guards in the virtual coordinates is the set $\mathcal{G}_v := \{G_v \subseteq \mathbb{R}^n: \exists \ i\geq 0, G_v = \gamma_{p_i}(Guard(p_i)) \}$.

The idea is to check what parts of $\mathcal{K}_v$ are actually possible modes initial sets. This can be done by 

We union all the tubes that we compute that 


\begin{corollary}
Let $\mathcal{G}_a = \{  \}$ 
\end{corollary}

$\cup_{\mathcal{G}_v} G_v$ in the corollary can be precomputed from the description of the graph. Moreover, the union of the initial sets starting from which we computed the reachtubes in the virtual coordinates can be stored in a variable and updated after each computation of a reachtube of a segment along with the intersection. 

\end{comment}




==> verif_algo.tex <==
%!TEX root = main.tex


\section{Symmetry-based verification algorithm}
\label{sec:unboundedsafety}
%\chuchu{
In this section, we introduce a novel safety verification algorithm, $\symsafety$, which uses existing reachability subroutines, but exploits symmetry, unlike existing algorithms. 
%Unlike existing algorithms which compute the reachtubes of multi-agent systems from scratch for each agent and each mode, $\symsafety$ reuses the reachtubes computed from the virtual system. As we have discussed, transforming reachtubes is more  efficient than computing reachtubes. Therefore, $\symsafety$ can speed up  verification while preserving the soundness and precision of the reachability subroutines.
%}
%\chuchu{
	In our earlier work~\cite{Sibai:ATVA2019}, we introduced  reachtube transformations using symmetry reduction for dynamical systems (Single mode). Here, we extend the method across modes and we introduce using the virtual system, and we develop the corresponding verification  algorithm.
%}

In Section~\ref{sec:tubecache_definition}, we define $\tubecache$---a data-structure for storing reachtubes; in~\ref{sec:symcompute}, we present the symmetry-based reachtube computation algorithm $\symcompute$ that resuses reachtubes stored in $\tubecache$; finally, in~\ref{sec:boundedtimesafety}, we define the $\safetycache$ data-structure which stores previously computed safety verification results which are used by the $\symsafety$ algorithm.
%\sout{In this section, we consider a scenario where multiple reachtubes of different modes, initial sets, and time bounds need to be computed. Such a scenario would be, for example, safety verification or controller synthesis of hybrid automata \cite{Fan_linear_control_syn_2018,C2E2paper,CAS13,breachAD}. Current algorithms and tools to handle such scenarios would compute each of these tubes from scratch. None of the tubes would be reused to compute others. In our recent work \cite{Sibai:ATVA2019}, reachtubes of a single mode are transformed to get ones of the same mode using equivariance and symmetry properties, but not to get reachtubes of a different mode.
%}

%\chuchu{Chuchu: It will be helpful to give a short overview of the overall algorithm here. Like, we first define $\tubecache, which ...$}
\subsection{$\tubecache$: shared memory for reachtubes}
\label{sec:tubecache_definition}
We show how we use the virtual system~(\ref{sys:virtual}) to create a shared memory for the different modes of the real system~(\ref{sys:input}) to reuse each others' computed reachtubes.
%
We call this shared memory $\tubecache$. 
%It stores reachtubes, as the  over-approximation of reachsets, of the virtual system~(\ref{sys:virtual}).
% \chuchu{
%	Later on, when dealing with the reachtube of the real systems, we will only need to transform the reachtubes in $\tubecache$ instead of computing the reachtubes again.
%} \sout{These reachtubes start from different initial sets and have potentially different time bounds.}

\begin{definition}
A $\tubecache$ is a data structure that stores a set of reachtubes of the virtual system~(\ref{sys:virtual}). It has two methods: $\mathit{getTube}$, for retrieving stored tubes and $\mathit{storeTube}$, for storing a newly computed one.
\end{definition}

 Given an initial set $K$, 
 %\chuchu{
 	we want to avoid computing the reachtube for it for as large portion of $K$ as possible.  Therefore,
% } 
$\mathtt{getTube}$ would return a list of reachtubes 
%\chuchu{
$\ARtube(K_i, p_v, [0,T_i]), i \in [k]$, for some $k \in \mathbb{N}$ that are already stored in $\tubecache$. Moreover, the union of $K_i$s is the largest subset of $K$ that can be covered by the initial sets of the reachtubes in $\tubecache$.
%}
 Formally,
\begin{align}
\label{def:tubecache}
\tubecache.\mathtt{getTube}(K) = \argmax_{\{\mathit{\ARtube(K_i,p_v, [0,T_i]) \in \tubecache\}_i}} \mathit{\text{Vol}(K \cap \cup_i {K_i})},
\end{align}
where $\mathit{\text{Vol}(\cdot)}$ is the Lebesgue measure of the set.
Note that for any $K \subset \mathbb{R}^n$, a maximizer of (\ref{def:tubecache}) would be the set of all reachtubes in $\tubecache$. However, this is very inefficient and the the union of all reachtubes in $\tubecache$ would be too conservative to be useful for checking safety. Therefore, $\mathtt{getTube}$ should return the minimum number of reachtubes that maximize~(\ref{def:tubecache}). 
%\chuchu{
Note that the reachtubes  in $ \tubecache$ may have different time bounds. We will truncate or extend them when used.
%}
%We present a simple such algorithm that approximates the optimal one in the next section.
\subsection{$\symcompute$: symmetry-based reachtube computation}
\label{sec:symcompute}

%\sout{Fix a method $\mathtt{computeReachtube}$ that computes reachtubes.  or corresponding overapproximations, for the real system~(\ref{sys:input}),  }

%\chuchu{
Given an initial set $K \subset S$, a mode $p \in P$, and time bound $T > 0$, there are dozen of tools that tools that can return a $\ARtube(K,p,[0,T])$. See \cite{C2E2paper,CAS13,breachAD} for examples of such tools. We denote this procedure by  $\tubecompute(K,p,[0,T])$. 
%}

%\chuchu{
	Compared with calling  $\mathtt{computeReachtube}(\cdot)$, whenever we need a reachtube, we want to use symmetry to reduce the load of computing new reachtubes by retrieving reachtubes that are already stored in $\tubecache$.
%}
  We introduce Algorithm~\ref{code:sym_annotations} which implements this idea and denote it by $\symcompute$. %\sout{Whenever a reachtube is needed with initial set $K$, mode $p$, and time bound $T$, we call $\symcompute$ instead of directly calling $\mathit{computeReachtube}$.} 
  We map the initial set $K$ to an initial set $K_v$ using $\gamma_p$, i.e. $K_v = \gamma_p(K)$, where the subscript $v$ for ``virtual''. Then, we map the resulting reachtube from the call back using $\gamma_p^{-1}$.
% For simplicity, $\tubecache$ that the initial sets of the tubes that $\tubecache$ stores are disjoint. 




%Moreover, consider the case where an algorithm call $\mathit{computeReachtube}$ several times with different arguments.

The input of $\symcompute$ consists of $K_v$ and $T$, and the $\tubecache$ that stores already computed reachtubes of the virtual system (\ref{sys:virtual}). %\sout{that resulted from previous calls.} 

%First, it would transform the initial set $K$ using $\gamma_p$ to get the corresponding initial set $K_v$ for the virtual system~(\ref{sys:virtual}) in line~\ref{ln:transformK}. 
First, it initializes $\mathit{restube}_v$ as an empty tube of the virtual system~(\ref{sys:virtual}) to store the result in line~\ref{ln:initialize_restube}. 
%
It then gets the reachtubes from $\tubecache$ that corresponds to $K_v$ using the $\mathtt{getTube}$ method in line~\ref{ln:gettube}. Now that it has the relevant tubes $\mathit{storedtubes}$, it adjusts their lengths based on the time bound $T$. For a retrieved tube with a time bound less than $T$ in line~\ref{ln:if_shorter}, $\symcompute$ extends the tube for the remaining time using $\tubecompute$ in lines~\ref{ln:extend_tube1}-\ref{ln:extend_tube2}, store the resulting tube in $\tubecache$ instead of the shorter one in line~\ref{ln:storetube}. If the retrieved tube is longer than $T$ (line~\ref{ln:if_longer}), it trims it in line~\ref{ln:trimtube}. However, we keep the long one in the $\tubecache$ to not lose a computation we already did. Then, the tube with the adjusted length is added to the result tube $\mathit{restube}_v$ in line~\ref{ln:unionres}.

The union of the initial sets of the tubes retrieved $\mathit{storedtubes}$ may not contain all of the initial set $K_v$. That uncovered part is called $K_v'$ in line~\ref{ln:remK}. The reachtube starting from $K_v'$ would be computed from scratch using $\tubecompute$ in line ~\ref{ln:compute_remtube}, stored in $\tubecache$ in line~\ref{ln:store_remtube}, and added to $\mathit{restube}_v$ in line~\ref{ln:union_remtube}. The resulting tube of the virtual system~(\ref{sys:virtual}) is returned in line~\ref{ln:return_tuberes}. This tube would be transformed by the calling algorithm using $\gamma_p^{-1}$ to get the corresponding tube of the real system~(\ref{sys:virtual}).
% Finally, using Theorem~\ref{thm:tube_trans_input}, the reachtube $\mathit{restube}$ is transformed back using $\gamma_p^{-1}$ in line~\ref{ln:transformres} to get the reachtube of mode $p$ starting from $K$ and running for $T$ time units.




\begin{algorithm}
	\small
	% : Symmetry annotation for reachtube computations
	\caption{$\symcompute$}
	\label{code:sym_annotations}
	%\begin{algorithm}	
	\begin{algorithmic}[1]
		\State \textbf{input:} $K_v, T, \tubecache$
		%\State $K_v \gets \gamma_p(K)$ \label{ln:transformK}
		\State $\mathit{restube}_v \gets \emptyset$ \label{ln:initialize_restube}
		\State $\mathit{storedtubes} \gets \tubecache.\mathtt{getTube}(K_v)$ \label{ln:gettube}
		\For{$i \in [|\mathit{storedtubes}|]$} \label{ln:for_loop_fixtubelength}
		\If{$\mathit{storedtubes}[i].T < T$} \label{ln:if_shorter}
		\State $(K_i,[\tau_{i-1}, T_i]) \gets \mathit{storedtubes}[i].\mathit{end}$ \label{ln:extend_tube1}
		\State $\mathit{tube}_i \gets \mathit{storedtubes}[i] \concat \tubecompute(K_i, p_v, [0,T - T_i])$ \label{ln:extend_tube2}
		\State $\tubecache.\mathtt{storeTube} (\mathit{tube}_i)$ \label{ln:storetube}
		\ElsIf{$\mathit{storedtubes}[i].T > T$}   \label{ln:if_longer}
		\State $\mathit{tube}_i \gets \mathit{storedtubes}[i].\mathit{truncate}(T)$ \label{ln:trimtube}
		\EndIf
		\State $\mathit{restube}_v \gets \mathit{restube}_v \cup tube_i$ \label{ln:unionres}
		\EndFor
		\State $K_{v}' \gets K_v \textbackslash \cup_i \mathit{storedtubes}[i].K$ \label{ln:remK}
		\State $\mathit{tube}' = \tubecompute(K_v', p_v, [0,T])$ \label{ln:compute_remtube}
		\State $\tubecache.\mathtt{storeTube} (\mathit{tube}')$  \label{ln:store_remtube}
		\State $\mathit{restube}_v \gets \mathit{restube}_v \cup \mathit{tube}'$ \label{ln:union_remtube}
		%\State $\mathit{result} \gets \gamma_p^{-1} (\mathit{restube}_v)$ \label{ln:transformres}
		\State \textbf{return:} {$\mathit{restube}_v$} \label{ln:return_tuberes}
	\end{algorithmic}
\end{algorithm}

\begin{theorem}
	\label{thm:tube_comp_alg_sound}
The output of Algorithm~\ref{code:sym_annotations} is an over-approximation of the reachtube $\Rtube(K_v,p_v,[0,T])$.
\end{theorem}
\begin{proof}
%\chuchu{
$\tubecompute$ always return over-approximations of the reachset from a given initial set and time bound, and $\mathit{restube}$ contains reachtubes that were computed by $\tubecompute$  at some point. 
%starting from $K_v'$ and having a time bound of $T$ is an over-approximation of $\Rtube(K_v',p_v,T)$ by assumption. Moreover, all the tubes in $\mathit{storedtubes}$ that are returned by $\tubecache.\mathit{getTube}$ are also computed by $\tubecompute$ in previous runs. Hence, they are over-approximations of the reachtubes starting from their corresponding initial sets.
There are three types of reachtubes in $\mathit{restube}$:
\begin{enumerate}
\item When the time bound $T_i$ of the stored reachtube $\mathit{storedtubes}[i]$ is less than $T$, we need to extend $\mathit{storedtubes}[i]$ until time $T$ by concatenating the original tube by $\tubecompute(K_i, p_v, [0,T - T_i])$  where $[K_i, [\tau_{i-1},T_i]$ is the last pair in $\mathit{storedtubes}[i]$. It is easy to check that the concatenated two reachtubes is a valid $(\mathit{storedtubes}[i].K, p_v, [0,T])$- reachtube.
\item When the time bound $T_i$ of the stored reachtube $\mathit{storedtubes}[i]$ is more than $T$, the truncated reachtube is also a valid  $(\mathit{storedtubes}[i].K, p_v, [0,T])$- reachtube.
\item For $K'_v$ that is not contained in the union of the initial sets in $\mathit{storedtubes}$, $\tubecompute$  will return a valid $(K'_v, p_v, [0,T])$- reachtube.
 Finally, the union of reachtubes is a reachtube of the union of the initial sets.
\end{enumerate}
The union of the initial sets of the tubes in $\mathit{storedtubes}$ and $K_v'$ contains $K_v$, so the union of the reachtubes  the algorithm returns a $(K_v, p_v, [0,T])$- reachtube.
%}
\end{proof}

The importance of $\symcompute$ lies in that if a mode $p$ required a computation of a reachtube and the result is saved in $\tubecache$, another mode with a similar scenario with respect to the virtual system would reuse that tube instead of computing one from scratch. Moreover, reachtubes of the same mode might be reused as well if the scenario was repeated again. 

%The following corollary shows that transforming the initial set of the mode $p$ that we compute the reachtube for using $\gamma_p$, providing it to $\symcompute$ and then transforming the result back using $\gamma_p^{-1}$ results in an over-approximated tube. It follows from Theorem~\ref{thm:tube_comp_alg_sound} and Corollary~\ref{cor:virtual_reachtube}.
%\begin{corollary}
%Fix a $\tubecache$, an initial set $K$, mode $p \in P$, time bound $T$. Then, $\Rtube(K,p,T) \subseteq \gamma_p^{-1}(\symcompute(\mathit{\gamma_p(K), T, \tubecache}))$.
%\end{corollary}

\subsection{Bounded time safety }
\label{sec:boundedtimesafety}

In this section, we show how to use $\tubecache$ and $\symcompute$ of the previous section for bounded and unbounded time safety verification of the real system~(\ref{sys:input}). We consider a scenario where the safety verification of multiple modes of the real system~(\ref{sys:input}) starting from different initial sets and for different time horizons is needed. We will use the virtual system~(\ref{sys:virtual}) and the transformations $\{\gamma_p\}_{p \in P}$ to share safety computations across modes, initial sets, time horizons, and unsafe sets.

 We first introduce $\safetycache$, a shared memory to store the results of intersecting reachtubes of the virtual system~(\ref{sys:virtual}) with different unsafe sets. It will prevent repeating safety checking computations of different modes under similar scenarios and can be used in finding unbounded time safety properties of the real system~(\ref{sys:input}).


\begin{definition}
	A $\safetycache$ is a data structure that stores the results of intersecting reachtubes of the virtual system~(\ref{sys:virtual}) with unsafe sets. It has two functions: $\mathtt{getIntersect}$, for retrieving stored results and $\mathtt{storeIntersect}$, for storing a newly computed one.
\end{definition}


Given an initial set $K_v$, a time bound $T$, and an unsafe set $U_v$, the reachtube $\AReach(K_v, p_v, [0,T])$ is going to be unsafe if another reachtubes $\AReach(K'_v, p_v, [0,T'])$ which is already stored  in $\tubecache$ is unsafe, and $\AReach(K'_v, p_v, [0,T'])$ is an under-approximation of $\AReach(K_v, p_v, [0,T])$. Similarly, if $\AReach(K'_v, p_v, [0,T'])$ is an over-approximation of $\AReach(K_v, p_v, [0,T])$ and is safe, then  $\AReach(K_v, p_v, [0,T])$ is safe.
Formally, the $\mathtt{getIntersect}$ function of $\safetycache$ returns the truth value of the predicate $\ARtube(K_v,p_v,[0,T]) \cap U_v \neq \emptyset$ if a subsuming computation is stored, and returns $\bot$, otherwise. 
%Formally, $\safetycache: 2^{\mathbb{R}^n} \times \mathbb{R}^+ \times 2^{\mathbb{R}^m} \rightarrow \{0,1,\bot\}$. 

Formally, $\safetycache.\mathtt{getIntersect}(K_v,T,U_v) =$
\begin{align*}
\begin{cases}
0, \text{ if } \exists K_v',T', U_v'\ |\ K_v \supseteq K_v', T\geq T', U_v \supseteq U_v', (K_v',T',U_v') \in \safetycache, \mathit{rtube} \cap U_v \neq \emptyset, \\
1, \text{ if } \exists K_v',T', U_v'\ |\ K_v \subseteq K_v', T\leq T', U_v \subseteq U_v', (K_v',T',U_v') \in \safetycache, \mathit{rtube} \cap U_v = \emptyset, \\
\bot, \text{ otherwise,}
\end{cases}
\end{align*}
where $\mathit{rtube} = \ARtube(K_v',p_v, [0,T'])$, $0$ means $\unsafe$, $1$, $\safe$, and $\bot$, not stored.


It is equivalent to check the intersection of a reachtube of the real system~(\ref{sys:input}) with an unsafe set $U$ and to check the intersection of the corresponding mapped reachtube and unsafe set of the virtual one. This is formalized in the following lemma.% which follow from the invertibility of the considered transformations. % $\gamma_p$, for all $p \in P$.  

%First, fix a mode $p$. We can check the safety of a reachtube of mode $p$ by mapping the unsafe set using $\gamma_p$ and checking the intersection of the resulting set with the corresponding reachtube in $\tubecache$.  
\begin{lemma}
	\label{lm:equiv_vir_real}
	Consider an unsafe set $U \subseteq \mathbb{R}^n \times \mathbb{R}^+$ and an over-approximated reachtube $\rtube = \ARtube(K,p,[t_1,t_2])$. Then, for any invertible $\gamma: \mathbb{R}^n \rightarrow \mathbb{R}^n$, $\mathit{rtube} \cap U \neq \emptyset$ if and only if $\gamma(\mathit{rtube}) \cap \gamma(U) \neq \emptyset$.
\end{lemma}
%\begin{proof}
	%If $\ARtube \cap U \neq \emptyset$ then $\exists\ x \in \ARtube \cap U$ and $\gamma(x) \in \gamma(\ARtube \cap U) = \gamma(\ARtube) \cap \gamma(U)$. Hence, $\gamma(\ARtube) \cap \gamma(U) \neq \emptyset$.
	%On the other hand, if $\gamma(\ARtube) \cap \gamma(U) \neq \emptyset$, then $\exists\ x \in \gamma(\ARtube) \cap \gamma(U)$ and $\gamma^-1(x) \in \gamma^-1( \gamma(\ARtube) \cap \gamma(U)) = \ARtube \cap U$.
%\end{proof}
	
Now that we have established the equivalence of safety checking between the real and virtual systems, we present Algorithm~\ref{code:sym_safety} denoted by $\symsafety$. It uses $\safetycache$, $\tubecache$, and $\symcompute$ in order to share safety verification computations across modes. The method $\symsafety$ would be called several times to check safety of different scenarios and $\safetycache$ and $\tubecache$ would be maintained across calls.

$\symsafety$ takes as input an initial set $K$, a mode $p$, a time bound $T$, an unsafe set $U$, the transformation $\gamma_p$, and $\safetycache$ and $\tubecache$ that resulted from previous runs of the algorithm.

It starts by transforming the initial and unsafe sets $K$ and $U$ to a virtual system initial and unsafe sets $K_v$ and $U_v$ using $\gamma_p$ in line~\ref{ln:transformK_s}. It then checks if a subsuming result of the safety check for the tuple $(K_v,T,U_v)$ exists in $\safetycache$ using its method $\mathtt{getIntersect}$ in line~\ref{ln:getintersect}. If it does exist, it returns it directly in line~\ref{ln:resreturn}. Otherwise, the approximate reachtube is computed using $\symcompute$ in line~\ref{ln:symcomputetube}. The returned tube is intersected with $U_v$ in line~\ref{ln:intersecttubeunsafe} and the result of the intersection is stored in $\safetycache$ in line~\ref{ln:saveresult}. It is returned in line~\ref{ln:resreturn}.





\begin{algorithm}
	\small
	% : Symmetry annotation for reachtube computations
	\caption{$\symsafety$}
	\label{code:sym_safety}
	%\begin{algorithm}	
	\begin{algorithmic}[1]
		\State \textbf{input:} $K, p, T, U, \gamma_p, \safetycache, \tubecache$
		\State $K_v \gets \gamma_p(K)$, $U_v \gets \gamma_p(U)$ \label{ln:transformK_s} 
		\State $\mathit{result} \gets \safetycache.\mathtt{getIntersect}(K_v,T,U_v)$ \label{ln:getintersect}
		\If{$\mathit{result} = \bot$}
		\State $\rtube \gets \symcompute$ $(K_v, T,\tubecache)$ \label{ln:symcomputetube}
		\State $\mathit{result} \gets (\mathit{tube} \cap U_v = \emptyset)$ \label{ln:intersecttubeunsafe}
		\State $\safetycache.\mathtt{storeIntersect}(K_v,T,U_v, result)$ \label{ln:saveresult}
		\EndIf
		\State \textbf{return:} {$\mathit{result}$}\label{ln:resreturn}
	\end{algorithmic}
\end{algorithm}

The following theorem show $\symsafety$ is able to prove safety.
\begin{theorem}
 If $\symsafety$ returns $\safe$, then $\Rtube(K,p,[0,T]) \cap U = \emptyset$.
\end{theorem}
\begin{proof}
From Theorem~\ref{thm:tube_comp_alg_sound}, if the result is not stored in $\safetycache$, we know that $\rtube$ in line~\ref{ln:symcomputetube} is an over-approximation of $\Rtube(K_v,p_v,[0,T])$. Moreover, we know from Corollary~\ref{cor:virtual_reachtube} that $\Rtube(K,p,[0,T]) \subseteq \gamma_p^{-1}(\rtube)$. But, from Lemma~\ref{lm:equiv_vir_real}, we know that the truth value of the predicate $(\rtube \cap U_v = \emptyset)$ is equal to that of $(\gamma_p^{-1}(\rtube) \cap U = \emptyset)$ and hence $\mathit{result}$ is $\safe$ if $\gamma_p^{-1}(\rtube) \cap U = \emptyset$ and thus it is $\safe$ if $\Rtube(K,p,T) \cap U = \emptyset$. Finally, the stored values in $\safetycache$ are results from previous runs, and hence have the same property. 
\end{proof}

However, if $\symsafety$ returns $\unsafe$, it might be that $\rtube$ in line~\ref{ln:symcomputetube} intersected the unsafe set because of an over-approximation error. There are two sources of such errors: the $\tubecompute$ method using by $\symcompute$ can itself result in over-approximation errors and actually it will most of the time~\cite{C2E2paper,CAS13}. But it may be exact too~\cite{bak2017hylaa}. The other source of errors is the $\tubecache.\mathtt{getTube}$ method which would return list of tubes with the union of their initial sets containing states that do not belong to the asked initial set. The first problem can be solved by: asking the method $\tubecompute$ to compute tighter reachtubes as existing methods provide this option for more computation~\cite{C2E2paper,CAS13}. We can use symmetry in these tightening computations as well as we did in \cite{Sibai:ATVA2019}. We can also replace saved tubes in $\tubecache$ with newly computed tighter ones.
The second problem can be solved by asking $\tubecache.\mathtt{getTube}$ to return only the tubes with initial sets that are fully contained in the asked initial set. This would decrease the savings from transforming cached results, but it would reduce the false-positive error, saying $\unsafe$ while it is $\safe$.





\subsection{Unbounded time safety}

In this section, we show how can we deduce unbounded safety checks results from finite ones. 
%We start by showing that from a single reachtube intersection with an unsafe set, we can deduce a safety check result  for every mode $p \in P$ that correspond to the same scenario.
The following corollary applies Lemma~\ref{lm:equiv_vir_real} to the transformations $\{\gamma_p\}_{p\in P}$ that map the different modes of the real system~(\ref{sys:input}) to the unique virtual one~(\ref{sys:virtual}).

\begin{corollary}[Infinite safety verification results from a single one]
	\label{cor:vir_real_eq_inter}
	Fix $U \subseteq \mathbb{R}^n$ and $\mathit{rtube} = \ARtube(K_v,p_v,[0,T]) $. If $\mathit{rtube} \cap U = \emptyset$, then for all $p \in P$, $\gamma_p^{-1}(\mathit{rtube}) \cap \gamma_p^{-1}(U) = \emptyset$.
\end{corollary}

The corollary means that from single reachtube $\ARtube(K,p_v,[0,T])$ and unsafe set $U$ intersection operation, we can deduce the safety of any mode $p$ starting from $\gamma_p^{-1}(K)$ and running for $T$ time units with respect to $\gamma_p^{-1}(U)$. This would for example imply unbounded time safety of a hybrid automaton under the assumption that the unsafe sets of the modes are at the same relative position with respect to the reachtube. But, $\safetycache$ stores a number of results of such operations. We can infer from each one of them the safety of infinite scenarios in every mode. This is formalized in the following theorem which follows directly from Corollary~\ref{cor:vir_real_eq_inter}.

\begin{theorem}[Infinite safety verification results from finite ones]
\label{thm:unboundedsafety}
For any mode $p \in P$, initial set $K \subseteq S$, time bound $T \geq 0,$ and unsafe set $U \subset S \times \mathbb{R}^{\geq 0}$, such that $K \subseteq \gamma_p^{-1}(K')$, $U \subseteq \gamma_p^{-1}(U')$, and $\safetycache(K',T,U') = 1$, system (\ref{sys:input}) is safe. 
\end{theorem}

As more saved results are added to $\safetycache$, we can deduce the safety of more scenarios in all modes. If at a given point of time, we are sure that no new scenarios would appear, we can deduce the safety for unbounded time and unbounded number of agents with the same dynamics having scenarios already covered.
%\begin{corollary}[Unbounded Safety]
%Given a $\tubecache$ and $\safetycache$, then if there is an algorithm 
%\end{corollary}



%\chuchu{Chuchu: I will wait until the examples are polished.}
\begin{example}[Fixed-wing aircraft infinite number of safety verification results from computing a single one]
\label{sec:inf_safetychecks_example}
Consider the initial set $K$, mode $p$, time bound $T$, and their corresponding virtual ones $K_v$ and $p_v$ considered in Example~\ref{sec:virtual_tube_example}. Let the unsafe set be $U = [[0, -\infty, 11.9,5.1],[\infty, \infty, 12.9, 6.1]] \times \mathbb{R}^{\geq 0}$ and $U_v = \gamma_{p_r}(U)$, where $\gamma_{p_r}$ is as described in Example~\ref{sec:virtual_tube_example}. Assume that $\rtube_v \cap U_v = \emptyset$ and the result is stored in $\safetycache$. Then, for all $p \in P$, $\gamma_p^{-1}(\rtube_v) \cap \gamma_p^{-1}(U_v) = \emptyset$.

%Fix a $\safetycache$ for the virtual system described in Example~\ref{sec:virtual_example} containing the result of intersecting the reachtube of the virtual system described in Example~\ref{sec:virtual_tube_example} with $U_v = \gamma_{p_r}(U)$. Assume that the intersection is empty.
For the aircraft, $U$ could represent a building. Crashing with the building at any speed, heading angle, and time is unsafe. $U_v$ represents the relative position of the building with respect to the segment of waypoints.
Theorem~\ref{thm:unboundedsafety} says that for any initial set of states $K$ of the aircraft and time bound $T$, if the relative positions of the aircraft, unsafe set, and the segment of waypoints are the same or subsumed by those of $K_v$, $U_v$, and the origin, we can infer safety irrespective of their absolute positions.
\end{example}

\begin{example}[Fixed-wing aircraft unbounded time safety]
\label{sec:unbounded_example}
Consider a sequence of modes $ p_0 = [0,0,10,0], p_1 = [10,0,10,10]$, $p_3 = [10,10, 0,10]$, $p_4 = [0,10,0,20]$, $p_5 = [0,20,20,20], p_6 = [20,20,20,30] \dots $ in $P$ which draw a vertical concatenations of $S$ shaped paths with segments of size 10. Assume that the aircraft in Example~\ref{sec:single_drone_example} switches between different modes once its position $[\state[2], \state[3]]$ is in the square with side equal to $1$ around the destination waypoint $[p_i[2],p_i[3]]$, the absolute value of the angle with the segment is at most $\frac{\pi}{6}$, and its speed within $0.5$ of $v_c$. We call this the $\mathit{guard}(p_i)$. Moreover, we assume that for each waypoint, there exists a corresponding unsafe set $U_{p_i} = [[0, -\infty, b_1,b_2],[\infty,\infty,u_1,u_2]]$, where the square $[[b_1,b_2],[u_1,u_2]]$ has radius 1 and center 2 units to the left of the center of the segment of $p_i$. One would verify the safety of such a system by computing the reachtube $\rtube_{p_i}$ of a mode $p_i$ and checking if it is safe by intersecting with $U_{p_i}$. If it is safe, we compute the intersection of $\rtube_{p_i}$ with $\mathit{guard}(p_i)$ to get the initial set for $p_{i+1}$, and repeat the process again. However, we know that the initial set of any mode $p_i$ is at most $\mathit{guard}(p_i)$ which we know its relative position with respect to the segment. Moreover, we know the position of the unsafe set with respect to the segment. Then, one can deduce the unbounded-time safety of this system by just checking the safety of one segment as all scenarios are the same in the virtual system.

\end{example}

%Consider the fixed-wing aircraft agent described in Section~\ref{sec:single_drone_example} and the corresponding transformation described in Section~\ref{}.

\begin{comment}

- mention why we added the source waypoint and its benefit in getting a statement about the angle between the segments between the waypoints for unbounded time safety.

- mention how we reached a fixed point if all the new states are transformed versions of each other.

- add more agents

- relative positions between agents, unsafe sets
\end{comment}


\begin{comment}
\section{Verification algorithm}
\label{sec:verification}
\vspace{-0.1in}

- intersection with the guard, what should we assume about the guard?

- existence of transformations of inputs that map them to unique input

- caching based algorithm (reachtube computation is abstracted away)

- dynamic and static safety checking.
\section{Experiments}

- four cases: using our own reachtube computer (C2E2, DryVR) with symmetry, without symmetry, and flow* computer with our symmetry, direct flow*

- examples: linear, dubin's vehicle, drone, 3d drone

- scenarios: keep unboundedness in mind (after the 5th agent no more computations are needed)
\end{comment}




==> verif_algo_multiple_gamma.tex <==
\subsection{The $\multiplesymtree$ procedure}
\label{sec:verification_Gamma}
\vspace{-0.1in}

Procedure $\multiplesymtree$ (Algorithm~\ref{code:symmetry_Gamma}) is a generalization of $\symtree$ using a group of symmetries. The $\multiplesymtree$ procedure still does BFS over $\cachTree$, keeps track of the parts of the input initial set $\initialset_n$ that are not proven safe  (line~\ref{ln:leftstatesupdate_m}); returns $\auto{Unsafe}$ with the same logic (line~\ref{ln:sym_unsafe_m}), and return $\auto{Compute}$ in case there are parts of $\initialset_n$ that are not proven safe nor have refinements in $\cachTree$ (line~\ref{ln:compute_m}). 

The key difference from $\symtree$ is that different transformations may be useful at different nodes. This leads to the possibility of multiple nodes in $\cachTree$, that are not ancestors or descendants of each other, covering the same parts of $\initialset_n$ under different transformations. Recall that in $\symtree$, only ancestors cover the parts of $\initialset_n$ that are covered by their descendants since $\gamma$ is invertible. Hence, it was sufficient to not add the children of a node to $\traversalstack$ to know that the part it covers, by transforming its initial set, from $\initialset_n$ is safe (line~\ref{ln:NoIntersect}). However, it is not sufficient in $\multiplesymtree$ since there may be another node that cover the same part of $\initialset_n$ which has a transformed reachtube that intersects $U$, hence refining what already has been proven to be safe. The solution is to remove explicitly from $\initialset_n$ what has been proven to be safe (line~\ref{ln:leftstatesupdate_m}). 
Moreover, it cannot return $\auto{Compute}$ when the transformed reachtube of a visited node intersects $U$ and its children initial sets do not contain the part it covers from $\initialset_n$ as in line~\ref{ln:compute} of $\symtree$. That is because other nodes may cover that part because of the availability of multiple symmetries. Hence, it cannot return $\auto{Compute}$ unless it traversed the whole tree and still parts of $\initialset_n$ could not be proven to be safe.
%\vspace{-.3in}
\vspace{-0.1in}
\begin{algorithm}
	\small
	\caption{$\multiplesymtree$}
	$\label{code:symmetry_Gamma}$
	\begin{algorithmic}[1]
		\State \textbf{input:} $\unsafe$, $\Gamma$, $\cachTree$, $\initialset_n$
		\State $\initialset_c := \cachTree.\rootnode.\initialset$
		%\State $\Gamma \gets getGamma(\initialset_c,\initialset_n)$
		%\State $\theta_u := \coverstack.\stacktop.\theta$ \Comment{new initial set with uncomputed reachtube}
		%\State $\delta_u := \coverstack.\stacktop.\delta$
		\If {$ \initialset_n \not\subseteq\cup_{\gamma \in \Gamma} \gamma (\initialset_c)$ $\label{al2:if_m}$}
		\State \textbf{return:} $\auto{SymmetryNotUseful}$ \label{ln:symNotUseful_m}
		\EndIf
		\State $\leftstates \gets \initialset_n$
		%\State $\tempstack := \{\langle \theta_u,\delta_u, \epsilon_u\rangle\}$
		\State $\traversalstack := \{\cachTree.\rootnode\}$
		\While {$\traversalstack \neq \emptyset$ and $\leftstates \neq \emptyset$}\label{ln:while_symtree_m}
		\State $\node \gets \traversalstack.dequeue()$ \label{ln:dequeue_m}
		\State $\initialset_c := \node.\initialset$; $\{(R_i,t_i)_{i=0}^k\} = \node.sim$
		%\State $\Gamma \gets getGamma(\initialset_c, \initialset_n)$
		\State $X = \{x  : \exists \gamma \in \Gamma, x \in \gamma (\initialset_c ) \text{ and } \gamma (\node.\overrt) \cap U = \emptyset \}$ \label{ln:computingX_m}
		\State $\leftstates \gets \leftstates \textbackslash X$ \label{ln:leftstatesupdate_m}
		\If{$\exists \gamma \in \Gamma, j\ |\ \gamma (R_j)\ \cap \ U \neq \emptyset \text{ and } \gamma (R_0) \in \leftstates$} \label{ln:if_unsafe_m}
		\State Return $\auto{Unsafe}$ \label{ln:sym_unsafe_m}
		%\Elsif{$|\node.\nodechildren| < 2^n$}
		%\State
		\EndIf
		\If{$len(\node.\nodechildren) > 0$}
		\State $\traversalstack.enqueue(\node.\nodechildren)$ \label{ln:addChildren_m}
		\EndIf
		\EndWhile
		\If {$\leftstates \neq \emptyset$} \label{ln:if_not_empty_m}
		\State \bf{return:} $\auto{Compute}$ \label{ln:compute_m}
		\EndIf
		\State \textbf{return:} $\auto{Safe}$ \label{ln:sym_safe_m}
		%\algstore{myalg}
	\end{algorithmic}
\end{algorithm}
\vspace{-0.2in}
We show that $\multiplesymtree$ has the same guarantees as $\symtree$ in the following two theorems with the proof being in Appendix~\ref{sec:app_symtree_proofs_m}.
\begin{restatable}[Completeness]{theorem}{secondcompleteness}
	\label{thm:termination_m}
	If there exists a set of nodes $S$ in $\cachTree$, where each $s\in S$ has a corresponding set of transformations $\Gamma_s \subseteq \Gamma$, such that
	\vspace{-0.1in} 
	\[\initialset_n \subseteq \cup_{s \in S, \gamma_s \in \Gamma_s} \gamma_s(s.\initialset) \text{ and } U \cap \cup_{s \in S, \gamma_s \in \Gamma_s} \gamma_s(s.\overrt) = \emptyset,\] 
	$\symtree$ will return ${\sf{Safe}}$. Also, if there exists a $\node$ $s$ in $\cachTree$ and a $\gamma \in \Gamma$, where $\gamma(s.sim)$ intersects $U$ and starts from $\initialset_n$, then $\multiplesymtree$ will return $\auto{SymmetryNotUseful}$, ${\sf{Unsafe}}$, or ${\sf{Compute}}$.
\end{restatable}
\vspace{-0.1in} 
\begin{restatable}[Soundness]{theorem}{secondsoundness}
	\label{thm:sym-reach-sound_m}
 $\multiplesymtree$ is sound: if it returns ${\sf{Safe}}$, then the reachtube $\Rtube(\initialset_n,T)$ does not intersect $U$ and if it returns ${\sf{Unsafe}}$, then there exists a trajectory starting from $\initialset_n$ that enters the unsafe set. 
\end{restatable}



The new challenge in $\multiplesymtree$ is in computing the union at line~\ref{al2:if_m}, computing $X$ in line~\ref{ln:computingX_m} and in the $\exists$ in line \ref{ln:if_unsafe_m}. These operations depend on $\Gamma$ if it is finite or infinite and how easy is to search over it. We revisit the arbitrary translation from Section~\ref{sec:symmetry:cps} to show that these operations are easy to compute in some cases.
\vspace{-0.1in}

\subsection{Revisiting arbitrary translations}
\label{sec:rev_arbitrary_trans}
Recall that the car model in example~\ref{eg:car_trans} in Section~\ref{sec:symmetry:cps} is equivariant to all translations in its position. In this section, we show how to apply $\multiplesymtree$ not just for it, but to arbitrary differential equations. Let $D$ be the set of components of the states that do not appear on the RHS of (\ref{eq:goal_ode}) and $\Gamma$ be the set of all translations of the components in $D$. To check the $\mathit{if}$ condition at line~\ref{al2:if_m}, we only have to check if $\initialset_c$ projected to the $[n] \textbackslash D$ contains $\initialset_n$ projected to the same components. Since if it is true, $\initialset_c$ can be translated arbitrarily in its components in $D$ so that the union contains $\initialset_n$.


%Moreover, if $\initialset_n$ and all $\initialset$s in $\cachTree$ are projected to $[n] \textbackslash D$, then running $\multiplesymtree$ will be equivalent to that of $\symtree$ with $\gamma$ being the identity map. That is because all maps in $\Gamma$ in this example change only the components that belong to $D$, and if these variables are removed by projection, all the maps become the identity map.  

Given two initial sets $K$ and $K'$ and the reachtube starting from $K'$, we compute $\beta \subseteq \mathbb{R}^n$ such that $K'\downarrow_D \oplus \beta = K \downarrow_D$. Then, if $K \subseteq K'$, by Corollary~\ref{cor:reachtube_transform}, we can use that $\beta$ to compute an overapproximation of $\Rtube(K,T)$ by computing $\Rtube(K',T) \oplus \beta$. Then, let $\beta$ be such that $\initialset_c\downarrow_D \oplus \beta = \leftstates\downarrow_D$, in line~\ref{ln:computingX_m}. 
%If $\node.rt \oplus \beta$ intersects $U$, we will need to refine.
 We set $X$ to be equal to $\initialset_c \oplus \beta$ if $\node.rt \oplus \beta \cap U = \emptyset$ and to $\emptyset$, otherwise.
 %
 To check the $\exists$ operator in line~\ref{ln:if_unsafe_m}, we can treat the simulation as $\node.rt$ and compute $\beta$ accordingly. Then, compute $\node.sim \oplus \beta$. The new condition would be then: if $R_j \oplus \beta \cap U$. Notice that we dropped $\gamma(R_0) \in \leftstates$ from the condition since we know that $R_0 \in \leftstates$ and $\beta$ is bloating it to the extent it is equal to $\leftstates$. 
 \vspace{-0.1in}
 
 \paragraph{Optimized $\multiplesymtree$ for arbitrary translations}
 
 The size of $K'\downarrow_D$ above does not matter, i.e. even if it is just a point, one can compute $\beta$ so that it covers $K\downarrow_D$. Hence, instead of computing $\Rtube(K,T)$, we compute only $\Rtube(K',T)$ and then compute $\beta$ from $K$ and $K'$ and then bloat it. This decreases the number of dimensions that the system need to refine by $|D|$. This is in contrast with what is done in $\multiplesymtree$ where the reachtubes are computed without changing the initial set structure. This improvement resulted in verifying models in 1s when they take an hour on DryVR as shown in Section~\ref{sec:experiments}. We call this algorithm $\transoptimized$ and refer to it as version 2 of $\multiplesymtree$ when applied to arbitrary translation invariance transformations. 
 
 %Moreover, if $\initialset_n$ and all $\initialset$s in $\cachTree$ are projected to $[n] \textbackslash D$, then running $\multiplesymtree$ will be equivalent to that of $\symtree$ with $\gamma$ being the identity map. That is because all maps in $\Gamma$ in this example change only the components that belong to $D$, and if these variables are removed by projection, all the maps become the identity map. 
%Notice that for after removing $X$ from $\leftstates$ in line~\ref{ln:leftstatesupdate_m}, none of the components of $\leftstates$ in $[n]\textbackslash D$ would be affected since $\Gamma$ only modify components in $D$. So, if the refinement is happening in one of the components in $[n] \textbackslash D$,  
%If the refinement was in one of the components in $D$, then the projection of the initial set to $[n]\textbackslash D$ would not change. Both the current node and the refined one would be able to cover $\initialset_n \downarrow_D$. Hence, it is correct to set $X$ to $\emptyset$ since the child (refined) node will have a tighter reachtube, after adding $\beta$, of that of its parent.

% There is no reason to set $X$ to a part of $\initialset_c \oplus \beta$ since any $\initialset$ of a $\node$ in $\cachTree$ would cover the $\initialset_n$ in the components in $D$.

% to check the safety of the system starting from an initial set $K$, we can compute the reachtube of the system starting from a new initial set $K'$ that has a projection to the components in $[n]\textbackslash D$ equal to that of $K$ and is a point when projected to the components in $D$. Then, we get $\beta$ such that $K' \oplus \beta = K$. We use this $\beta$ to compute $\Rtube(K,T)$ by computing $\Rtube(K',T) \oplus \beta$. Then, we can refine in the components in $[n]\textbackslash D$ to get tighter reachtubes since the tube is the tightest possible in the components in $D$. 
%We call this method the {\sf fast} one. 


%The projection $\initialset_c \downarrow_D$ of $\initialset_c$ to the components in $D$ is a hyperrectangle. The projection $\leftstates\downarrow_D$ of $\leftstates$ to the components in $D$ is compact. Hence, there exists a finite number of translations of $\initialset_c \downarrow_D$ that have a union that covers $\initialset_n \downarrow_D$. To compute $X$ at line~\ref{ln:computingX_m}, we check which of these translations when applied to $\node.rt$ do not intersect $U$. The union of the corresponding translated initial sets is $X$. This may leave some states that are safe from being part of $X$ because there might be multiple sets of translations that cover $\leftstates$. This will make $\multiplesymtree$ return $\auto{Compute}$ more. 
%However, if $\initialset_c\downarrow_D$ is a point we define $\gamma^*$ to be the map as well just translate $\initialset_c$ to be at the center of $\leftstates$ and 

%To check the $\mathit{if}$ condition at line~\ref{ln:if_unsafe_m}, we define the translation and bloating map $\gamma^*$ to be the one that takes $R_0$ to a set of states that when projected to $D$ is equal to $\leftstates\downarrow_D$ and leaves all other dimensions unaltered. Then, we apply $\gamma^*$ to $R_j$, for all $j \in [k]$. If any intersects $U$, then it is $\auto{Unsafe}$.

%Note that we do not have to compute the reachtube from the whole given initial set $K$. We can consider instead $K'$ which when projected on $[n]\textbackslash D$ is equal to the projection of $K$ on the same components while it is a single point when projected on the components in $D$. Then, we can rely on $\Gamma$ to cover $K$ in line~\ref{al2:if_m} and to compute $X$ in line~\ref{ln:computingX_m}. This will decrease the dimensions that need refinement by $|D|$.

\begin{comment}

Let $\gamma^*$ be a map that translates $\initialset_n$ to the center of $\leftstates$ and makes its projection to the components in $D$ equal to that of $\leftstates$ when projected on the same components. Then, $X$ is equal to $\gamma^*(\initialset_c)$ if $\gamma^*(\node.rt) \cap U = \emptyset$, and equal to $\emptyset$, otherwise.
 We let $X$ at line~\ref{ln:computingX_m} to be equal to $\gamma(\initialset_c)$


Before discussing how to compute $X$ at line~\ref{ln:computingX_m} and check the $\mathit{if}$ condition at line~\ref{ln:if_unsafe_m}, we consider a simpler problem.
%Consider two axes aligned hyperrectangles $K_1$ and $K_2 \subset \mathbb{R}^n$ representing two initial sets of states. 
Assume that the projection of $\initialset_c$ to the components in $D$ is a point.
%and that we already computed the reachtube of the system starting from it.  
Then, if we want to use the computed reachtube to get as much as we can from the reachtube starting from $K_2$, we grid the box in $K_2$ that correspond to these variables with diameters equal to the diameters of $K_1$. On the boundaries, the cells of the grid may overlap but no extra states should be covered because of the griding. After that, we compute the translation vector that takes the center of $K_1$ to the center of each cell in the grid.  Then, we use these vectors to translate the computed reachtube and union them to get a reachtube for $K_2$. However, there might be exponential number of grid cells and we will need to translate the reachtube exponential number of times. This will slow computation and computing reachtube in the usual way may be faster.

To solve this issue, we define the following map $\gamma_b : X \rightarrow X'$. 
$\gamma_b$ takes a bounding box $X \subset \mathbb{R}^n$ as input and returns a bounding box $X'$. First, it translates $X$ by the difference between the center of $K_2$ from the center of $K_1$. Then, it adds to the upper bound in $X$ of a dimension $d$ that is translation invariant the difference between the upper bound of $K_2$ with the upper bound of the translated $K_1$, if the difference is positive, and adds to the lower bound the difference between the corresponding lower bounds, if the difference is negative.

%we may translate $K_1$ to the center of $K_2$ and then bloat the lower and upper bound of each translation invariant dimension to contain that of $K_2$. This is equivalent to translating $K_1$ several times above.
The following theorem relates the result of translating the reachtube that starts from $K_1$ several times and unioning the result as described above with applying $\gamma_b$ to the reachtube starting from $K_1$.
\begin{theorem} Let $\Gamma_g$ be the set of translations that move $K_1$ to the centers of the grid in $K_2$ and $\gamma_b$ be the transformation that translate $K_1$ to the center of $K_2$ and then increase the upper bound of the translated $K_1$ of each translation invariant dimension to match that of $K_2$ and decrease the corresponding lower bound similarly. Then,
	\[
	\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \Rtube(\gamma_b(K_1), T) = \gamma_b(\Rtube(K_1,T)).
	\]
	Moreover, $\Rtube(\gamma_b(K_1), T) \supseteq \Rtube(K_2, T)$.
\end{theorem} 
\begin{proof}
	Note first that $\gamma_b(K_1) = \cup_{\gamma \in \Gamma_g} \gamma(K_1) \supseteq K_2$. Moreover, we know that $\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \Rtube(\cup_{\gamma \in \Gamma_g} \gamma(K_1), T)$. Hence, the first equality. Also, by Theorem~\ref{thm:reachtube_transform}, $\Rtube(\gamma(K_1), T) = \gamma(\Rtube(K_1, T))$, for all $\gamma \in \Gamma_g$. Hence, $\cup_{\gamma \in \Gamma_g}\Rtube(\gamma(K_1), T) = \cup_{\gamma \in \Gamma_g}\gamma (\Rtube(K_1, T)) = \gamma_b (\Rtube(K_1, T))$. Therefore, $\gamma_b (\Rtube(K_1, T)) = \Rtube(\gamma_b(K_1), T)$. Finally, since $\gamma_b(K_1) \supseteq K_2$, the last inequality follows.
\end{proof}

\end{comment}
\vspace{-.1in}





==> verif_algo_thms.tex <==
\begin{restatable}[Completeness]{theorem}{firstcompleteness}
	\label{thm:termination}
	If there exists a set of nodes $S$ in $\cachTree$ with \[\initialset_n \subseteq \cup_{s \in S} \gamma(s.\initialset) \text{ and } U \cap \cup_{s \in S} \gamma(s.\overrt) = \emptyset,\] $\symtree$ will return ${\sf{Safe}}$. Also, if there exists a $\node$ $s$ in $\cachTree$ where $\gamma(s.sim) \cap U \neq \emptyset$ and starts from $\initialset_n$, then $\symtree$ will return $\auto{SymmetryNotUseful}$, ${\sf{Unsafe}}$, or ${\sf{Compute}}$.
\end{restatable}

\begin{comment}
\begin{proof}
We will prove the ${\sf{Safe}}$ and ${\sf{Unsafe}}$ cases separately. But first, note that $\symtree$ traverses $\cachTree$ in a BFS manner and $\cachTree$ is of finite size. Hence, $\symtree$ terminates. 
\paragraph{${\sf{Safe}}$} %The condition in the theorem implies that $U \cap \gamma(\node.\overrt) = \emptyset$ for all $\node \in S$. Moreover, the while loop at line~\ref{ln:while_symtree} traverses $\cachTree$ in a BFS manner. Hence, if any of these nodes got visited, i.e. dequeued at line~\ref{ln:dequeue}, the condition at line~\ref{ln:if_safe} will be true. That means that $\symtree$ will not return ${\sf{Unsafe}}$ or ${\sf{Compute}}$ in that iteration and none of its children will be enqueued in $\traversalstack$. 

First, the $\initialset$ of the root contains all the $\initialset$s in the tree. Hence, if the union of the transformation of the $\initialset$s of the nodes in $S$ under $\gamma$ contains $\initialset_n$, then so does $\gamma(\rootnode.\initialset)$. Then, $\symtree$ will not return $\auto{SymmetryNotUseful}$.

Second, we prove that $\symtree$ will not return ${\sf{Unsafe}}$. Assume that the condition at line~\ref{ln:if_unsafe} was taken at a given iteration where some node $\node_p$ is the one being visited. Then, $\gamma(\node_p.sim)$ starts from $\initialset_n$ and intersects $U$. By Theorem~\ref{thm:reachtube_transform}, this is a simulation of the system that starts from $\gamma(\node_p.sim.R_0)$.  However, by the assumption of the current theorem, there exists a $\node_c \in S$ with $\node.\initialset_c$ that contains $\gamma(\node_p.sim.R_0)$. Moreover, from Definition~\ref{def:discrepancy} and $\simVerif$, we know that simulation belongs to $\node_c.\overrt$. But, $\node_c.\overrt \cap U = \emptyset$, contradiction. Hence, the condition at line~\ref{ln:cond_addChildren} could not be taken under the assumptions of the theorem.

%Moreover, if some $\node \in S$ was never visited in the while loop, that means that its parent or one of its grandparents in $\cachTree$ was visited in some iteration and the condition at line~\ref{ln:cond_addChildren} was not taken in that iteration. Let us name that parent or grandparent $\node_p$. 

Third, we will prove that $\symtree$ will not return ${\sf{Compute}}$. Assume for the sake of contradiction that it returned ${\sf{Compute}}$ at a given iteration and $\node_p$ was the node being visited. Then, all the conditions in the while loop were not satisfied. Hence, there exists subset $\gamma(\node_p.\initialset) \cap \initialset_n$ that is not covered by the transformed initial sets of the children of $\node_p$. Since $\gamma$ is inveritble and the initial sets of the children  are disjoint, then that part would not be covered by other nodes in the tree other than $\node_p$ and its parent and grandparents. However, all of these parent nodes have $\overrt$ that intersect $U$ for them to got refined in the first place. Hence, none of them belong to $S$. Therefore, there is no node in $S$ with $\initialset$ that cover that part. That contradicts our assumption that the union of $\initialset$s of nodes in $S$ contains $\initialset_n$. Therefore, $\symtree$ does not return ${\sf{Compute}}$ under the assumptions of the theorem.

Finally, since the algorithm terminates and it would not return ${\sf{Compute}}$, ${\sf{Unsafe}}$, or $\auto{SymmetryNotUseful}$, it will return ${\sf{Safe}}$.

\paragraph{${\sf{Unsafe}}$} Let $\node_p$ be a node in $\cachTree$ with $\gamma(\node.sim)$ that starts from $\initialset_n$ and intersects $U$. Then, in the BFS traversal of $\cachTree$, for none of its parent and grandparents, the condition at line~\ref{ln:if_safe} will be true since $\node.sim \subseteq \node.\overrt$. Hence, $\symtree$ will either return ${\sf{Compute}}$, ${\sf{Unsafe}}$, or $\auto{SymmetryNotUseful}$ before visiting $\node_p$ or it will visit it and line~\ref{ln:if_unsafe} will be true. In that case, $\symtree$ will return ${\sf{Unsafe}}$.
\end{proof}
\end{comment}

\begin{restatable}[Soundness]{theorem}{firstsoundness}
	\label{thm:sym-reach-sound}
	$\symtree$ is sound: if it returns ${\sf{Safe}}$, then the reachtube $\Rtube(\initialset_n,T)$ does not intersect $U$ 
	 and if it returns ${\sf{Unsafe}}$, then there exists a trajectory starting from $\initialset_n$ that enters the unsafe set. 
\end{restatable}

\begin{comment}
\begin{proof}
	We will again separate the proofs for the ${\sf{Safe}}$ and ${\sf{Unsafe}}$ cases.
	\paragraph{${\sf{Safe}}$} If $\symtree$ returns ${\sf{Safe}}$, it means that the condition in line~\ref{al2:if} is not true. Moreover, in every iteration of the while loop, either the condition in line~\ref{ln:if_safe} or the one in line~\ref{ln:cond_addChildren} is taken. When the one in line~\ref{ln:if_safe} is taken, it means either that the node is useless for computing the reachtube starting from $\initialset_n$ or the reachtube does not intersect $U$. If the condition at line~\ref{ln:cond_addChildren} was taken, it adds children with union of the transformed $\initialset$s cover the part of $\initialset_n$ that was covered by the parent $\initialset$. Hence, none of the states in $\initialset_n$ will not be checked the safety for. Thus, every state in $\initialset_n$ will belong to some $\node.\initialset$ for which line~\ref{ln:if_safe} will be true. Therefore, the system starting from $\initialset_n$ is safe.
	\paragraph{${\sf{Unsafe}}$} Assume that the node visited in the iteration at which $\symtree$ returned ${\sf{Unsafe}}$ be $\node_p$. Then, $\gamma(\node_p.\sim)$ starts from $\initialset_n$ and intersects $U$. Moreover, by Theorem~\ref{thm:sol_transform}, it is the simulation of the system starting from $\node_p.\sim.R_0$. Hence, it is a counter example and the system is unsafe.                                                                                                                                                           
\end{proof}
\end{comment}


In summary, $\symtree$ shows that a single symmetry $\gamma$ could decrease the number of fresh reachtube computations needed for verification. Next, we revisit  Example~\ref{eq:simplelinear} to illustrate the need for multiple symmetry maps.


\paragraph{Circular orbits and scaling symmetry}
The linear system in Example~\ref{eq:simplelinear} has circular orbits. Consider the initial set $K = [[21.5,21.5],[24.5,24.5]]$, 
%where the first list represent the lower bounds for $x_1$ and $x_2$ and the second one, their upper bounds respectively. 
the unsafe set $x_2 \geq 32$ after $t = 1.4s$, and the time bound $T=1.5s$. Any matrix $B$ that commutes with $A$, the RHS of the differential equation, is a symmetry transformation. However, once this matrix is fixed, we do not change it as per $\symtree$. Any diagonal matrix that commutes with $A$ has equal diagonal elements. Such a matrix would scale $x_1$ and $x_2$ by the same factor. Hence, applying $B$ to any axis aligned box would either scale the box up or down on the diagonal. That means applying $B$ to $K$ wouldn't contain the upper left or bottom right partitions, but only possibly the bottom left corner. With  $B = [[0.95,0], [0, 0.95]]$, only one out of 7 reachtubes is obtained via transformation (first row of Table~\ref{table:experimental_results}). 

That is because we are using a single transform which leaves $\symtree$ in most of the input cases useless. Figure~\ref{fig:circle_nosym} shows the reachtube (colored green to  yellow) computed using $\simVerif$, unsafe set (brown). Figure~\ref{fig:circle_sym} shows the reachtube computed using $\simVerif$ and $\symtree$. The part of the reachtube that was computed using symmetry is colored between blue and violet.
The other part is still between yellow and green. Only the upper left corner has been transformed instead if being computed. Next, we present $\multiplesymtree$, a generalization of $\symtree$ that uses a group of symmetries aiming for a bigger ratio of transformed to computed reachtubes.

\vspace{-0.3in}


